Learning Overcomplete HMMs

We study the problem of learning overcomplete HMMs---those that have many hidden states but a small output alphabet. Despite having significant practical importance, such HMMs are poorly understood with no known positive or negative results for efficient learning. In this paper, we present several new results---both positive and negative---which help define the boundaries between the tractable and intractable settings. Specifically, we show positive results for a large subclass of HMMs whose transition matrices are sparse, well-conditioned, and have small probability mass on short cycles. On the other hand, we show that learning is impossible given only a polynomial number of samples for HMMs with a small output alphabet and whose transition matrices are random regular graphs with large degree. We also discuss these results in the context of learning HMMs which can capture long-term dependencies.

==> NIPS Arxiv/abstract.tex <==
\vspace{-12pt}
\begin{abstract}
\vspace{-8pt}
We study the problem of learning overcomplete HMMs---those that have many hidden states but a small output alphabet. Despite having significant practical importance, such HMMs are poorly understood with no known positive or negative results for efficient learning. In this paper, we present several new results---both positive and negative---which help define the boundaries between the tractable and intractable settings. Specifically, we show positive results for a large subclass of HMMs whose transition matrices are sparse, well-conditioned, and have small probability mass on short cycles.  On the other hand, we show that learning is impossible given only a polynomial number of samples for HMMs with a small output alphabet and whose transition matrices are random regular graphs with large degree. We also discuss these results in the context of learning HMMs which can capture long-term dependencies.
% We discuss these results in the context of learning HMMs with long-term dependencies.
%We study the problem of learning HMMs with many hidden states but a small output alphabet. For HMMs with a small output alphabet and whose transition matrices are random regular graphs with large degree, we show that learning is impossible given only a polynomial number of samples. We also show positive results for a large subclass of HMMs whose transition matrices are sparse, well-conditioned and have small probability mass on short cycles. We discuss these results in the context of learning HMMs with long-term dependencies.%, and show that our results imply that least some HMMs with long-term dependencies can be learned efficiently from short time windows.
\end{abstract}


==> NIPS Arxiv/conclusion_colt.tex <==
\vspace{-10pt}
\section{Conclusion and Future Work}\label{sec:conclusion}
% The setting where the output alphabet $m$ is much smaller than the number of hidden states $n$ is well-motivated in practice and seems to have several interesting theoretical questions about new lower bounds and algorithms. Though some of our results are obtained in more restrictive conditions than seems necessary, we hope the ideas and techniques pave the way for much sharper results for this setting. A better understanding of the memory and long range dependencies for HMMs in this regime would be especially interesting, and getting a better understanding of what properties of the transition and observation matrices lead to the output process having long-term dependencies would probably be insightful for both theory and practice. 
\vspace{-5pt}

The setting where the output alphabet $m$ is much smaller than the number of hidden states $n$ is well-motivated in practice and seems to have several interesting theoretical questions about new lower bounds and algorithms. Though some of our results are obtained in more restrictive conditions than seems necessary, we hope the ideas and techniques pave the way for much sharper results in this setting. Some open problems which we think might be particularly useful for improving our understanding is relaxing the condition on the observation matrix being random to some structural constraint on the observation matrix (such as on its Kruskal rank), and more thoroughly investigating the requirement for the transition matrix being sparse and not having short cycles.


%It is interesting to consider the implications of our results to sequential models beyond HMMs. Recently, many applications have demonstrated the superior ability of Long Short Term Memory (LSTM) \cite{hochreiter1997long} networks over Recurrent Neural Networks (RNNs) at capturing long term dependencies in  data. A RNN is a fully connected neural network where all the weights are unconstrained, whereas the weight matrix of a LSTM network is constrained to have certain sparse connections. Other models which either initialize the weight matrix of a RNN to be sparse \cite{le2015simple} or constrain it to be sparse \cite{mikolov2014learning}, have also had good success in learning long term dependencies. It would be interesting if sparsity in RNNs also leads to efficient learning, as we showed is the case for HMMs. We also hope that the ideas and techniques we introduced lead to sharper results for HMMs in the overcomplete setting, and close some of the gaps between the upper bounds and lower bounds.


% To summarize, the setting where the output alphabet $m$ is much smaller than the number of hidden states $n$ is well-motivated in practice, and seems to have several interesting theoretical questions about new lower bounds and algorithms. We hope that the ideas and techniques we introduce lead to sharper results in this setting, and close some of the gaps between the upper bounds and lower bounds.

% Though some of our results are obtained in more restrictive conditions than seems necessary, we hope the ideas and techniques pave the way for much sharper results for this setting.


% It would be interesting if sparsity in RNNs also leads to efficient learning, as it

%This points to some of our observations that sparse transition matrices both seem to be easier to learn, and are useful for capturing long term dependencies. 

%Our results also indicate that long-term  dependencies should not be hard to learn if we get generic observations about the current state. In essence, when the observations are generic, they leak some information about the current state at each time step, which makes it possible to learn these models over short windows. 
%\section{Conclusion}


==> NIPS Arxiv/identifiability_nips.tex <==
\vspace{-8pt}
\section{Identifiability of HMMs from short windows}\label{sec:identifiability}
\vspace{-8pt}
As it is not obvious that some of the requirements for Theorem \ref{thm:learnability} are necessary, it is natural to attempt to derive stronger results for just identifiability of HMMs having structured transition matrices. In this section, we state our results for identifiability of HMMs from windows of size $\Oh{\log_m n}$.  \citet{huang14hmm} showed that all HMMs except those belonging to a measure zero set become identifiable from windows of length $2\tau + 1$ with $\tau=8\lceil \log_m n\rceil$. However, the measure zero set itself might possibly contain interesting classes of HMMs (see Fig. \ref{fig:examples}), for example sparse HMMs also belong to a measure zero set. We refine the identifiability results in this section, and show that a natural sparsity condition on the transition matrix guarantees identifiability from short windows. Given any transition matrix $T$, we regard $T$ as being supported by a set of indices $\mathcal{S}$ if the non-zero entries of $T$ all lie in $\mathcal{S}$. We now state our result for identifiability of sparse HMMs.

\begin{restatable}{thm}{identifiability}\label{thm:identifiability}
  Let $\mathcal{S}$ be a set of indices which supports a permutation where all cycles have at least $2\lceil \log_m n \rceil$ hidden states. Then the set $\mathcal{T}$ of all transition matrices with support $\mathcal{S}$ is identifiable from windows of length $4\lceil \log_m n\rceil +1$ for all observation matrices $O$ except for a measure zero set of transition matrices in $\mathcal{T}$ and observation matrices $O$.
\end{restatable}
\noindent \emph{Proof sketch.} Recall from Section \ref{sec:technical_contri} that the main task is to show that the likelihood matrix $A$ is full rank. The proof uses basic algebraic geometry, and the main idea used is analogous to the following fact about polynomials: either a polynomial is a zero polynomial or it has finitely many roots which will lie in a measure zero set. The determinant of the likelihood matrix $A$ (or of sub-matrices of $A$ if $A$ is rectangular) is a polynomial in the entries of $T$ and $O$, hence we only need to show that the polynomial is not a zero polynomial. To show that a polynomial is not a zero polynomial, it is sufficient to find one instance of the variables which makes the polynomial non-zero. Hence we only need to find some particular $T$ and $O$ such that the determinant is not 0. We find such a $T$ and $O$ using the fact that $\mathcal{S}$ supports a permutation which does not have short cycles.\hfill $\square$

%\noindent \emph{Proof sketch.} Recall from Section \ref{sec:technical_contri} that the main task is to show that the likelihood matrix $A$ is full rank. The proof uses basic algebraic geometry, and the main idea used is analogous to the following fact about polynomials: either a polynomial is a zero polynomial or it has finitely many roots which will lie in a measure zero set. The determinant of the likelihood matrix $A$ (or of sub-matrices of $A$ if $A$ is rectangular) is a polynomial in the entries of $T$ and $O$, hence we only need to show that the polynomial is not a zero polynomial. To show that a polynomial is not a zero polynomial, it is sufficient to find one instance of the variables which makes the polynomial non-zero. Hence we only need to find some particular $T$ and $O$ such that the determinant is not 0. We find such a $T$ and $O$ using the fact that $\mathcal{S}$ supports a permutation which does not have short cycles.\hfill $\square$
%\vspace{-4pt}
%We remark that Proposition \ref{thm:identifiability} does allow the presence of short cycles in the graph, but cannot handle cases when the transition matrix is only composed of short cycles. 
\vspace{-4pt}
We hypothesize that excluding a measure zero set of transition matrices in Theorem \ref{thm:identifiability} should not be necessary as long as the transition matrix is full rank, but are unable to show this. Note that our result on identifiability is more flexible in allowing short cycles in transition matrices than Theorem \ref{thm:learnability}, and is closer to the lower bound on identifiability in Proposition \ref{lem:iden_lower_bnd}.

We also strengthen the result of \citet{huang14hmm} for identifiability of generic HMMs. \citet{huang14hmm} conjectured that windows of length $2\lceil \log_m n\rceil +1$ are sufficient for generic HMMs to be identifiable. The constant 2 is the information theoretic bound as an HMM on $n$ hidden states and $m$ outputs has $\Oh{n^2+nm}$ independent parameters, and hence needs observations over a window of size $2\lceil \log_m n\rceil +1$ to be uniquely identifiable. Proposition \ref{thm:special_identifiability} settles this conjecture, proving the optimal window length requirement for generic HMMs to be identifiable. As the number of possible outputs over a window of length $t$ is $m^t$, the size of the moment tensor in Section \ref{sec:technical_contri} is itself exponential in the window length. Therefore even a factor of 2 improvement in the window length requirement leads to a quadratic improvement in the sample and time complexity. %The proof is similar to the proof of Theorem \ref{thm:identifiability}.

\begin{restatable}{prop}{tightwindow}\label{thm:special_identifiability}
	The set of all HMMs is identifiable from observations over windows of length $2\lceil \log_m n\rceil +1$ except for a measure zero set of transition matrices $T$ and observation matrices $O$.
\end{restatable}


==> NIPS Arxiv/identifiability_proof_nips.tex <==
\section{Additional proofs for Section \ref{sec:identifiability}: Identifiability results}

\identifiability*
\begin{proof}
	We first show that the matrices $A$, $B$ and $A'=(O \odot A^{(\tau-1)})$ become full rank using observations over a window of length $N=2\tau +1$, where $\tau = 2 \lceil \log_m n \rceil$.
	
	Let's fix the window length to be $N=2\tau +1$, where $\tau = 2 \lceil \log_m n \rceil$.  We choose the transition matrix $T$ to be the permutation which is supported by $\mathcal{S}$. By the requirement in Theorem \ref{thm:identifiability}, $T$ is composed of cycles all of which have at least $\tau$ hidden states. Without loss of generality, assume that all cycles in $T$ are composed of sequences of hidden states $\{h_{i},h_{i+1},\dotsb,h_{j-1},h_{j}\}$ for $i,j \in [n], i\le j$. To further simplify notation we also assume, without loss of generality, that each cycle of $T$ is a cyclic shift of the hidden states $\{h_{i},h_{i+1},\dotsb,h_{j-1},h_{j}\}$.
	
	To show that $A,B$ and $A'$ are full rank, it is sufficient to show that they become full rank for some particular choice of $O$. Say that we choose each hidden state $h_i$ to always deterministically output some character $a_i$. We show that $A$ is full-rank for some assignment of outputs to hidden states. The same argument will also imply that $B$ and $A'$ are full rank. Because the transition matrix is a permutation, Markov chains starting in two different starting states are at different hidden states at every time step. Also, because all cycles in the permutation are longer than $\tau$, at every time step at least one of the two states visited by the two initial starting states has not been visited so far by either of the two initial starting states. Hence, the probability of the emissions corresponding to the two initial starting states being the same at any time step is $(1/m)$. Therefore, the probability that the emissions for two different hidden states across a $\tau$ length windows is the same is $(1/m)^{\lceil 2\log_m n \rceil}\le 1/n^2$. As the total number of pairs of hidden states is $n(n-1)/2$, by a union bound, the probability there exists some observation matrix such that the emissions for the $\lceil 2\log_m n \rceil$ window corresponding to all initial states are different is strictly great than 0. By choosing the $O$ which has this property, the matrix $A$ is full rank. By the same reasoning, $A'$ and $B$ are also full rank.

	Hence, as we have shown that there exists some transition matrix $T$ which is supported by $\mathcal{S}$ and observation matrix $O$ such that $A, A'$ and $B$ become full rank. Hence $A, A'$ and $B$ are full rank except for a measure zero set of $T$ and $O$. As the matrix $C$ is linearly independence except for a measure zero set of $O$, Kruskal's condition is satisfied except for a measure zero set of $T$ and $O$, and $A'$ is full rank, hence due to Algorithm \ref{alg:learn_tensor}, the set of HMMs is identifiable except for a measure zero set of $T$ and $O$. This concludes the proof.
	
\end{proof}

\tightwindow*
\begin{proof}
	The proof idea is similar to Theorem \ref{thm:identifiability}. We will choose some particular choice of $T$ and $O$ such that the matrices $A,B$ and $A'$ become full rank. Consider $T$ to be the permutation on $n$ hidden states which performs a cyclic shift of the hidden states i.e. $T_{ij}=1$ if $j=(i+1)\mod n$ for $0\le i,j\le k-1$ and $T_{ij}$ is 0 otherwise. We show that for this particular choice of $T$, there exists a choice of $O$ such that $A$ becomes full-rank for $t=\lceil \log_m n\rceil +1$. As in the proof of Proposition \ref{thm:identifiability}, we choose each hidden state to deterministically output a character, hence each column of $O$ has one non-zero entry. We show that $A$ is full-rank for some choice of $O$, the same argument will also imply that $B$ and $A'$ are full rank for that $O$.
	
	Because the transition matrix is a cyclic shift, we can reformulate the problem of finding a suitable $O$ as that of finding a length $n$ $m$-ary string all of whose length $\tau=\lceil \log_m n\rceil$ cyclic-substrings are unique (a substring is defined as a continuous subsequence), treating the string as cyclic so that the ends wrap around. De Bruijn sequences have exactly this property. A De Brujin sequence of length $k$ is a cyclic sequence in which every possible length $\lfloor \log_m k \rfloor$ $m$-ary string occurs exactly once as a substring. Furthermore, these sequences also have the property that all substrings longer than $\lfloor \log_m k \rfloor$ are unique \cite{flaxman2004strings}. Hence choosing a De Bruijn sequence of length $k=n$ ensures that all substrings of length $\lceil \log_m n\rceil \ge \lfloor \log_m n\rfloor$ are unique.
	
	Hence we have shown that there exists a choice of $O$ such that the matrix $A$ becomes full rank with windows of length $2\lceil \log_m n\rceil +1$ for some choice of $O$. Hence by the same argument as in the proof of Proposition \ref{thm:identifiability}, all HMMs except those belonging to a measure zero set of $T$ and $O$ become identifiable with windows of length $2\lceil \log_m n\rceil +1$.
\end{proof}

\idenbound*
	\begin{proof}
		There are $m^c$ possible outputs over a window of length $c$. Define a larger alphabet of size $m^c$ which denotes output sequences over a window of length $c$. Dividing the window of length $t$ into $t/c$ segments, the probability of a output sequence only depends on the counts of outputs from the larger alphabet and follows a multinomial distribution. The total number of possible counts is at most $\Big(\frac{2t}{c}\Big)^{m^c}$ as each of the $m^c$ outputs can have a count from 0 to $t/c$. Therefore windows of length $t$ give at most $\Big(\frac{2t}{c}\Big)^{m^c}$ independent measurements, hence the window length has to be at least $O(n^{1/{m^c}})$ for the model to be identifiable as an HMM has $O(n^2+nm)$ independent parameters.
	\end{proof}


==> NIPS Arxiv/intro_nips.tex <==
\vspace{-18pt}
\section{Introduction}
\vspace{-5pt}
Hidden Markov Models (HMMs) are commonly used for data with natural sequential structure (e.g., speech, language, video).
This paper focuses on \emph{overcomplete} HMMs, where the number of output symbols $m$ is much smaller than the number of hidden states $n$.
As an example, for an HMM that outputs natural language documents one character at a time, the number of characters $m$ is quite small, but the number of hidden states $n$ would need to be very large to encode the rich syntactic, semantic, and discourse structure of the document.

% The setting with many hidden states but a small output alphabet is also very relevant from the point of view of the important problem of modeling sequential data which has \emph{long-term dependencies}---defined as settings where observations from a long time window in the past are necessary for making a prediction about the future. The reason is that in the small output alphabet setting we only receive a small amount of information about the true hidden state at each step, and hence longer windows are necessary to infer the hidden state and make a good prediction. If the size of the output alphabet is instead comparable to the number of hidden states, then the outputs may provide a lot of information about the current hidden state at each time step. In this case, short windows are sufficient for correctly guessing the hidden state and hence predicting the next output to a high accuracy. 

Most algorithms for learning HMMs with provable guarantees
assume the transition $T \in \mathbb R^{n \times n}$ and observation $O \in \mathbb R^{m \times n}$ matrices are full rank \cite{anandkumar2012method,anandkumar13tensor,mossel2005learning} and hence do not apply to the overcomplete regime. A notable exception is the recent work of  \citet{huang14hmm} who studied this setting where $m \ll n$ and showed that \emph{generic} HMMs can be learned in polynomial time given \emph{exact} moments of the output process (which requires infinite data). Though understanding properties of generic HMMs is an important first step, in reality, HMMs with a large number of hidden states typically have structured, non-generic transition matrices---e.g., consider sparse transition matrices or transition matrices of factorial HMMs \cite{ghahramani1997factorial}. \citet{huang14hmm} also assume access to exact moments, which leaves open the question of when learning is possible with efficient sample complexity.
Summarizing, we are interested in the following questions:
%For the case where the transition and observation matrices are both full-rank, spectral methods via the method of moments are known to be able to efficiently recover the parameters of the HMM \cite{anandkumar2012method,anandkumar13tensor,mossel2005learning}. 

%In this setting, it is sufficient to obtain the moments of the process over a time window of length 3 to learn the parameters. However, constraining the observation matrix to be full-rank implies that the output alphabet $m$ is as large as the number of hidden states $n$. Despite its fundamental nature, much less is known about the overcomplete setting where the output alphabet is much smaller than the number of hidden states. In this case, windows of length 3 no longer suffice and we need to merge observations over longer time windows to learn the model. As the number of possible samples required to estimate moments over a window of length $t$ is $m^t$ for an output alphabet of size $m$, hence it is desirable to learn the model over the minimum window length possible for the method of moments based recovery. Here, by the window length required for learning, we mean the time window over which observations or moments are needed to learn the model.

%In this work, we aim to understand the learnability of overcomplete HMMs from short time windows. In recent work, \citet{huang14hmm} studied this setting where $m \ll n$ and showed that \emph{generic} HMMs become identifiable from windows of length $\Oh{\log_m n}$, and hence can be learned in polynomial time given \emph{exact} moments over a $\Oh{\log_m n}$ length window. Though this resolves the question of whether generic HMMs are identifiable from short windows, the overcomplete setting is far from understood. The following questions are long-standing and seem particularly pertinent--
\begin{enumerate}
	\item What are the fundamental limitations for learning overcomplete HMMs?
	\item What properties of HMMs make learning possible with polynomial samples?
	\item Are there structured HMMs which can be learned in the overcomplete regime?
\end{enumerate}

%As the previous work only deals with identifiability, it is not clear if and when learning is actually possible with polynomial samples. It is also pertinent to examine whether \emph{structured} HMMs which have interesting long-term behavior, rather than \emph{generic} HMMs, can be learned in this small output alphabet setting.  \\

%several questions still remain unanswered. Generic HMMs are rapid mixing and hence do not have any interesting long-term behavior, hence it seems pertinent to examine if more structured HMMs can be learnt in this setting. Also, even for generic HMMs, the sample complexity of learning the parameters has not been studied so far and it was not known when learning is actually possible with polynomial samples.\\
\vspace{-5pt}
\noindent \textbf{Our contributions.} We make progress on all three questions in this work, sharpening our understanding of the boundary between tractable and intractable learning. We begin by stating a negative result, which perhaps explains some of the difficulty of obtaining strong learning guarantees in the overcomplete setting.

%\medskip
\begin{thm}\label{thm:lower_bound}
	The parameters of HMMs where i) the transition matrix encodes a random walk on a regular graph on $n$ nodes with degree polynomial in $n$, ii) the output alphabet $m=\polylog{n}$ and, iii) the output distribution for each hidden state is chosen uniformly and independently at random, cannot be learned (even approximately) using polynomially many samples over any window length polynomial in $n$, with high probability over the choice of the observation matrix.
\end{thm}
%\noindent \textbf{Theorem ~\ref{thm:lower_bound}.} \emph{ HMMs where i) the transition matrix is a random walk on a regular graph on $n$ nodes with degree polynomial in $n$, ii) the output alphabet $m=\polylog{n}$ and iii) the output distribution for each hidden state is chosen uniformly and independently at random, cannot be learned using polynomially many samples over any window length polynomial in $n$, with high probability over the choice of the observation matrix.}
%\medskip
\vspace{-6pt}
Theorem \ref{thm:lower_bound} is somewhat surprising, as parameters of HMMs with such transition matrices can be easily learned in the non-overcomplete ($m \ge n$) regime. This is because such transition matrices are full-rank and their condition numbers are polynomial in $n$; hence spectral techniques such as \citet{anandkumar13tensor} can be applied. Theorem~\ref{thm:lower_bound} is also fundamentally of a different nature as compared to lower bounds based on parity with noise reductions for HMMs \cite{mossel2005learning}, as ours is information-theoretic.\footnote{Parity with noise is information theoretically easy given observations over a window of length at least the number of inputs to the parity. This is linear in the number of hidden states of the parity with noise HMM, whereas Theorem \ref{thm:lower_bound} says that the sample complexity must be super polynomial for any polynomial sized window.} Also, it seems far more damning as the hard cases are seemingly innocuous classes such as random walks on dense graphs. The lower bound also shows that analyzing generic or random HMMs might not be the right framework to consider in the overcomplete regime as these might not be learnable with polynomial samples even though they are identifiable. This further motivates the need for understanding HMMs with structured transition matrices. We provide a proof of Theorem \ref{thm:lower_bound} with more explicitly stated conditions in Appendix \ref{sec:lower_bound_proof}.

%We provide a proof sketch and formal proof of Theorem \ref{thm:lower_bound} in Section \ref{sec:lower_bound} Appendix \ref{sec:lower_bound_proof}.

%Hence the small output alphabet setting provides a separation between learnability of random, dense HMMs and structured HMMs. As such dense transition matrices are rapidly mixing (they mix in constant time) hence they are not very interesting from a prediction point of view either. Therefore, it appears that such models where prediction is easy are naturally excluded from the class of learnable HMMs in the setting where $m \ll n$. This provides additional motivation for studying the setting where $m \ll n$. We provide a sketch of the proof of Theorem \ref{thm:lower_bound} in Section \ref{sec:lower_bound}.

%An additional difficulty of the setting when $m \ll n$ is that some very simple models are not even identifiable from windows of length $\Oh{\log_m n}$. For example, consider an HMM with transition matrix $T=I$ and binary observations ($m=2$). In this case, the probability of output sequences follows the binomial distribution and only depends on the total number of zeros or ones in the sequence. Therefore, we only get $t$ independent measurements from windows of length $t$, hence windows of length $\Oh{n}$ instead of $\Oh{\log_2 n}$ are necessary for identifiability. More generally, we prove in Proposition \ref{lem:iden_lower_bnd} that a transition matrix composed only of cycles of constant length requires the window length to be polynomial in $n$ to become identifiable (see Fig. \ref{fig:cycle} for an example of such a transition matrix). This means that many seemingly simple transition matrices must be excluded from the class of models learnable from short windows.

%In light of these difficulties, it seems worthwhile to understand the problem of learning overcomplete HMMs from the perspective of properties of the transition matrix alone. Note that the observation matrix cannot be full rank in our overcomplete setup, and an adversarial choice for it can make even simple transition matrices such as a cycle impossible to learn with short windows (refer to Fig. \ref{fig:worsrt_O} for an example). 

% Our positive results on learnability aim to understand  To disentangle the additional complications due to the choice of the observation matrix, we will assume that the observation matrix is drawn at random throughout the paper. Long-standing open problems on learning \emph{aliased} HMMs (HMMs where some hidden states have identical output distributions) \cite{blackwell57identifiable,ito1992identifiability,weiss2015learning} hint that understanding learnability from the point of view of properties of the observation matrix is a daunting task in itself, and is perhaps best studied separately from the perspective of understanding how properties of the transition matrix affect learning.

%\begin{restatable}{thm}{learnability}\label{thm:learnability}
%	If an HMM satisfies the above conditions, then with high probability over the choice of $O$, the parameters of the HMM learnable to within additive error $\epsilon$ with observations over windows of length $2\tau +1, \tau = 15\log_m n$ with the sample complexity being $\poly{n,1/\epsilon}$.
	%If an HMM satisfies the above conditions with $\delta_1,\delta_2,\delta_3\le \delta \le 1/n^{c_1}$ for any constant $c_1>0$ and $ \sigma_{\min}^{(1)}(T),\sigma_{\min}^{(1)}(T') \ge 1/m^{c_1/2}$, then with high probability over the choice of $O$, the parameters of the HMM learnable to within additive error $\epsilon$ with observations over windows of length $2\tau +1, \tau = 20\log_m n$ with the sample complexity being $\poly{n,1/\epsilon}$.
%\end{restatable}

%\medskip
%\noindent \textbf{Theorem ~\ref{thm:learnability_l1}.} \emph{(Informal) If the transition matrix of the HMM is sparse (constant degree), well-conditioned (constant minimum singular value) and has small probability mass on cycles shorter than $10\log_m n$ states and the output distribution of each hidden state is random on a uniformly random support on the output alphabet, then with high probability the HMM can be learnt using observations from a $\Oh{\log_m n}$ window to within error $\epsilon$ using $\poly{n,1/\epsilon}$ samples.}
%\medskip
\vspace{-2pt}
For our positive results we focus on understanding properties of structured transition matrices which make learning tractable. To disentangle additional complications due to the choice of the observation matrix, we will assume that the observation matrix is drawn at random throughout the paper. Long-standing open problems on learning \emph{aliased} HMMs (HMMs where multiple hidden states have identical output distributions) \cite{blackwell57identifiable,ito1992identifiability,weiss2015learning} hint that understanding learnability with respect to properties of the observation matrix is a daunting task in itself, and is perhaps best studied separately from understanding how properties of the transition matrix affect learning.

Our positive result on learnability (Theorem \ref{thm:learnability}) depends on two natural graph-theoretic properties of the transition matrix. We consider transition matrices which are i) {sparse} (hidden states have constant degree) and ii) have small probability mass on cycles shorter than $10\log_m n$ states---and show that these HMMs can be learned efficiently using tensor decomposition and the method of moments, given random observation matrices. The condition prohibiting short cycles might seem mysterious. Intuitively, we need this condition to ensure that the Markov Chain visits a sufficient large portion of the state space in a short interval of time, and in fact the condition stems from information-theoretic considerations. We discuss these further in Sections~\ref{sec:examples} and \ref{subsec:assumptions}. We also discuss how our results relate to learning HMMs which capture long-term dependencies in their outputs, and introduce a new notion of how well an HMM captures long-term dependencies. These are discussed in Section \ref{sec:long_term}. 

%Fig. \ref{fig:example1} and \ref{fig:example2} illustrate some transition matrices which fit in our framework. Fig. \ref{fig:example1} represents a sparse transition matrix without short cycles, properties which we argued are relevant for language modeling. Fig. \ref{fig:example2} represents an HMM with a permutation as the transition matrix. Such an HMM can be thought of as a topic model with drift, which cycles through a large collection of topics. Section \ref{subsec:examples} explains why these HMMs can be learnt using our results, and provides some additional examples.

We also show new identifiability results for sparse HMMs. These results provide a finer picture of identifiability than \citet{huang14hmm}, as ours hold for sparse transition matrices which are not generic.

%\vspace{-1pt}
\noindent \textbf{Technical contribution.} To prove Theorem \ref{thm:learnability} we show that the Khatri-Rao product of dependent random vectors is well-conditioned under certain conditions. Previously, \citet{bhaskara2014smoothed} showed that the Khatri-Rao product of independent random vectors is well-conditioned to perform a smoothed analysis of tensor decomposition, their techniques however do not extend to the dependent case. For the dependent case, we show a similar result using a novel Markov chain coupling based argument which relates the condition number to the best coupling of output distributions of two random walks with disjoint starting distributions. The technique is outlined in Section \ref{sec:technical_contri}.

%\vspace{-5pt}
%\vspace{-1pt}
%\noindent \textbf{Motivating settings and applications.} Consider an HMM which approximates a generative model for language on a character level---this requires modeling significant long-term dependencies. The output at each time step is a character, and the latent state encodes any syntactic or semantic information. For example, the latent state would need to capture some very local information (for simple syntax--adjectives before nouns, etc.), track what entities have been mentioned (so that it can resolve anaphora--who does 'she' refer to) and any topic information (perhaps on different time scales--sections and subsections, etc). Such an HMM would have a very large latent space, but a small output alphabet. We can  expect the transition matrix of the HMM to be sparse, as most syntactic and semantic states will not co-occur with each other---for example most words in English hardly co-occur with each other. We might also reasonably expect the transition matrix to not have high probability mass on short cycles, as syntactic and semantic state will not recur very often---even though the word `HMM' repeats many times in this paper, the syntactic and semantic context is usually not the same. A model similar to language also holds for speech, where the output at every time step is a phoneme instead of a character. Hence HMMs with large, sparse transition matrices which do not have high probability mass on short cycles plausibly represent interesting classes of HMMs which can capture long term dependencies.
% We attempt to motivate our goal of understanding HMMs with large, sparse transition matrices which do not have high probability mass on short cycles. 

%\vspace{-1pt}
\noindent \textbf{Related work.} Spectral methods for learning HMMs have been studied in \citet{anandkumar13tensor,bhaskara13tensor,allman09identifiability,hsu2012spectral}, but these results require $m\ge n$. In \citet{allman09identifiability}, the authors show that that HMMs are identifiable given moments of continuous observations over a time interval of length $N=2\tau+1$ for some $\tau$ such that ${\tau+m-1 \choose m-1}\ge n$. When $m\ll n$ this requires $\tau=\Oh{n^{1/m}}$. \citet{bhaskara13tensor} give another bound on window size which requires $\tau=\Oh{n/m}$. However, with a output alphabet of size $m$, specifying all moments in a $N$ length continuous time interval requires $m^N$ time and samples, and therefore all of these approaches lead to exponential runtimes when $m$ is constant with respect to $n$. Also relevant is the work by \citet{anandkumar2015learning} on guarantees for learning certain latent variable models such as Gaussian mixtures in the overcomplete setting through tensor decomposition. As mentioned earlier, the work closest to ours is \citet{huang14hmm} who showed that generic HMMs are identifiable with $\tau=\Oh{\log_m n}$, which gives the first polynomial runtimes for the case when $m$ is constant.

%\pl{can cut to save space}
\noindent \textbf{Outline.} Section \ref{sec:setup} introduces the notation and setup. It also provides examples and a high-level overview of our proof approach. Section \ref{sec:learnability} states the learnability result, discusses our assumptions and HMMs which satisfy these assumptions. Section \ref{sec:identifiability} contains our identifiability results for sparse HMMs. Section \ref{sec:long_term} discusses natural measures of long-term dependencies in HMMs. We state the lower bound for learning dense, random HMMs in Section \ref{sec:lower_bound}. We conclude in Section \ref{sec:conclusion}. We provide proof sketches in the main body, rigorous proofs are deferred to the Appendix.  %Section \ref{sec:lower_bound} states the lower bound for learning dense, random HMMs. 

%\noindent \textbf{Outline:} The outline of the paper is as follows. In Section \ref{sec:related} we review some of the literature on learning HMMs with guarantees. In Section \ref{sec:examples} we provide some motivating examples of classes of HMMs which fit in our framework. We review notation and the general approach of learning HMMs using tensor decomposition in Section \ref{sec:setup}. In Section \ref{sec:identifiability} we discuss our results for identifiability of HMMs from short windows. Subsequently in Section \ref{sec:learnability} we discuss our results on learning HMMs with polynomial samples. Section \ref{sec:lower_bound} contains our lower bound for random, dense transition matrices. We conclude in Section \ref{sec:conclusion}.


==> NIPS Arxiv/learning_proof.tex <==
\section{Additional proofs for Section \ref{sec:learnability}: Learnability results}\label{sec:learning_proof}


\noindent \textbf{Assumptions for learning HMMs efficiently:}

For some fixed constants $c_1, c_2, c_3 > 1 $, the HMM should satisfy the following properties for some $c>0$:
\begin{enumerate}
	%	\item \emph{Markov Chain is stationary:} $T$ has a stationary distribution, and every hidden state has stationary probability at least $1/\poly{n}$.
	\item \emph{Transition matrix is well-conditioned:} Both $T$ and the transition matrix $T'$ of the time reversed Markov Chain are well-conditioned in the $\ell_1$-norm: $\sigma_{\min}^{(1)}(T),\sigma_{\min}^{(1)}(T') \ge 1/m^{ c/c_1}$%\footnote{$\sigma_{\min}^{(1)}(T)$ is defined as $\min_{x\in \mathbb{R}^n}\frac{\absnorm{Tx}}{\absnorm{x}}$. We also obtain slightly weaker results for }
	%We outline the conditions in Theorem \ref{thm:learnability_l1} and Corollary \ref{thm:learnability}.
	\item \emph{Transition matrix does not have short cycles:} For both $T$ and $T'$, every state visits at least $10 \log_m n$ states in $15 \log_m n$ time except with probability $\delta_1 \le 1/n^c$.
	%$\sigma_{\min}(T),\sigma_{\min}(T')>1/m^{1/20}$.
	\item \emph{All hidden states have small ``degree'':} There exists $\delta_2$ such that for every hidden state $i$, the transition distributions $T_i$ and $T'_i$ have cumulative mass at most $\delta_2$ on all but $d$ states, with $d \le m^{1/c_2}$ and $\delta_2 \le 1/n^c$. Hence this is a soft ``degree'' requirement.
	%The ``degree'' $d$ is the size of the minimum set such that the transition distributions $T_i$ and $T'_i$ have cumulative mass at most $\delta_2$ on all but $d$ states, with $d \le m^{1/c_2}$ and $\delta_2 \le 1/n^c$.
	%	There exists $\delta_2$ such that for every hidden state $i$, the transition distributions $T_i$ and $T'_i$ have cumulative mass at most $\delta_2$ on all but $d$ states, with $d \le m^{1/c_2}$ and $\delta_2 \le 1/n^c$.
	\item \emph{Output distributions are random and have small support:} There exists $\delta_3$ such that for every hidden state $i$ the output distribution $O_i$ has cumulative mass at most $\delta_3$ on all but $k$ outputs, with $k\le m^{1/c_3}$ and $\delta_3 \le 1/n^c$. Also, the output distribution $O_i$ is randomly chosen from the simplex on these $k$ outputs.
\end{enumerate}

%\begin{thm}\label{thm:learnability}
%		If an HMM satisfies the above conditions, then with high probability over the choice of $O$, the parameters of the HMM are learnable to within additive error $\epsilon$ with observations over windows of length $2\tau +1, \tau = 15\log_m n$, with the sample complexity being $\poly{n,1/\epsilon}$.
%\end{thm}
\learn*

\begin{proof}
	Let the window length $N=2\window+1$ where $\window = 15\log_m n$. We will prove the theorem for $c_1 = 20, c_2 = 16$ and $c_3 = 10$, these can be modified for different tradeoffs. By Lemma \ref{lem:jennrich} from \citet{bhaskara2014smoothed}, the simultaneous diagonalization procedure in Algorithm \ref{alg:learn_tensor} needs $\poly{n,1/\beta,\kappa,1/\epsilon}$ samples to ensure that the decomposition is accurate to an additive error $\epsilon$, with $\beta$ and $\kappa$ defined below.
	
	\begin{lem}\cite{bhaskara2014smoothed}\label{lem:jennrich}
		Suppose we are given a tensor $M+E\in \mathbb{R}^{m \times n \times p}$ with the entries of $E$ being bounded by $\epsilon=\poly{1/\kappa, 1/n, 1/\beta}$ and $M$ has a decomposition $M = \sum_{i=1}^{R}A_i \otimes B_i \otimes C_i$ which satisfies-
		\begin{enumerate}
			\item The condition numbers $\kappa(A), \kappa(B) \le \kappa$. 
			\item The column vectors of $C$ are not close to parallel: for all $i\ne j$, ${\largenorm{{\frac{w_i}{\norm{w_i}}-\frac{w_j}{\norm{w_j}}}} \ge \beta}$
			\item The decompositions are bounded: for all $i$, $\norm{u_i}, \norm{v_i}, \norm{w_i}\le K$
		\end{enumerate}
		then the simultaneous decomposition algorithm recovers each rank one term in the decomposition of $M$ (up to renaming), within an additive error of $\epsilon$.
	\end{lem}
	 
	Lemma \ref{lem:bound_dist} (proved in Section \ref{sec:lemma2}) shows that the observation matrix $O$ satisfies condition 2 in Lemma \ref{lem:jennrich} with $\beta = 1/n^{6.5}$.
	
	\begin{restatable}{lem}{bounddist}\label{lem:bound_dist}
		If each column of the observation matrix is uniformly random on a support of size $k$, then ${\norm{{\frac{O_i}{\norm{O_i}}-\frac{O_j}{\norm{O_j}}}} \ge 1/n^{6.5}}$ with high probability over the choice of $O$.
	\end{restatable}
	
	
	Note that as $A,B$ and $O$ are all stochastic matrices, all the factors have $\ell_2$ norm at most 1, therefore condition 3 in Lemma \ref{lem:jennrich} is satisfied with $K=1$. Hence if we show that the condition numbers $\kappa(A), \kappa(B)\le \poly{n}$, then each rank one term $A_i \otimes B_i \otimes C_i$ can be recovered up to an additive error of $\epsilon$ with $\poly{n,1/\epsilon}$ samples. As $\pi_i$ is at least $1/\poly{n}$ for all $i$, this implies that $A, B, C$ can be recovered with additive error $\epsilon$ with $\poly{n,1/\epsilon}$ samples. As $O$ can be recovered from $C$ by normalizing $C$ to have unit $\ell_1$ norm, hence $O$ can be recovered up to an additive error $\epsilon$ with $\poly{n, 1/\epsilon}$ samples. 
	
	If the estimate $\hat{A}$ of $A$ is accurate up to an additive error $\epsilon$, then the estimate $\hat{A}^{(\window-1)}$ of $A^{(\window-1)}$ is accurate up to an additive error $O(m\epsilon)$. Therefore, if the estimate $\hat{O}$ of $O$ is also accurate up to an additive error $\epsilon$ then the estimate of $\hat{A}'=(\hat{O}\odot \hat{A}^{(\window-1)})$ of $A'$ is accurate up to an additive error $O(n\epsilon)$. Further, if the matrix $A'$ also has condition number at most $\poly{n}$, then the transition matrix $T$ can be recovered using Algorithm \ref{alg:learn_tensor} with up to an additive error of $\epsilon$ with $\poly{n,1/\epsilon}$ samples. Hence we will now show that the condition number $\kappa(A)\le \poly{n}$. The proof for an upper bound for $\kappa(A')$ and $\kappa(B)$ follows by the same argument.
	
	Define the $(1-\delta)$-support of any distribution $p$ as the set such that $p$ has mass at most $\delta$ outside that set. For convenience, define $\delta=\max\{\delta_1, \delta_2, \delta_3\}$ in the conditions for Theorem \ref{thm:learnability}. We will find the probability that the Markov chains only undertakes transitions belonging to the  $(1-\delta)$-support of the current hidden state at each time step. As the probability of transitioning to any state outside the $(1-\delta)$-support of the current hidden state is at most $\delta$, and the transitions at each time step are independent conditioned on the hidden state, the probability that the Markov chains only undertakes transitions belonging to the $(1-\delta)$-support of all hidden state for each of the $n$ time steps is at least $(1-\delta)^{\window} \ge 1-{2\window}{\delta}$. \footnote{For $x \in [0,0.5], n>0, xn \le 1, (1-x)^n \in [1-2xn, 1-xn/2]$.}
	
	By the same argument, the probability of a sequence of hidden states always emitting an output which belongs to the $(1-\delta)$-support of the output distribution of the hidden state at that time step is at least $(1-\delta)^{\window}\ge 1-{2\window}{\delta}$.
	
	We now show that two sequences of hidden states which do not intersect have large distance between their output distributions. The output alphabet over a window of size $\tau$ has size $K=m^\window$. Let $\{a_i, i \in [K]\}$ be the set of all possible output in $\window$ time steps. For any sequence $s$ of hidden states over a time interval $\window$, define $o_{s}$ to be the vector of probabilities of output strings conditioned on any sequence of hidden states $s$, hence $o_{s} \in \mathbb{R}^{K}$ and the first entry of $o_s$ equals $P(a_1|s)$. Lemma \ref{determine} (proved in Section \ref{sec:lemma3}) shows that the output distributions of sample paths which do not meet in $\tau$ time steps is large with high probability.
	
	\begin{restatable}{lem}{determine}\label{determine}
		Let $s_i$ and $s_j$ be two sequences of $\window$ hidden states which do not intersect. Also assume that $s_i$ and $s_j$ have the property that the output distribution at every time step corresponds to the $(1-\delta)$ support of the hidden state at that time step. Let $o_{s_i}$ be the vector of probabilities of output strings conditioned on any sequence of hidden states $s_i$. Also, assume that $s_i$ and $s_j$ both visit at least $(1-\alpha) n$ different hidden states. Then, 
		\begin{align}
		P\Big[\absnorm{o_{s_i}-o_{s_j}} = 1\Big]\ge \Big(\frac{4m^2}{d}\Big)^{0.5(1-\alpha) \window}\nonumber
		\end{align}
		%Then $\Prob\Big[\absnorm{o_{s_i}-o_{s_j}} \ge 1-\frac{1}{k^{{c\alpha/2}}}\Big] \ge 1-1/k^{c\alpha}$. 
	\end{restatable}

	Note that $\alpha \le 1/3$ according to our condition 3 of Theorem \ref{thm:learnability}. Also, as $k<m^{1/10}$, therefore $\Big(\frac{4k^2}{m}\Big)^{ \window/3}\le (4/m^{4/5})^{\window/3}$. Now consider the set $\mathcal{M}$ of all sequences with the property that the transition at every time step corresponds to the $(1-\delta)$-support of the hidden state at that time step. As the $(1-\delta)$-support of every hidden state has size at most $d$, $|\mathcal{M}|\le nd^{\window}$. Now for a sequence $s_i$, consider the set $\mathcal{M}_{s_i}$ of all sequences $s_j$ which do not intersect that sequence. By a union bound---
	\begin{align}
	P\Big[\absnorm{o_{s_i}-o_{s_j}} = 1 \; \forall s_j \in \mathcal{M}_{s_i}\Big] \ge 1- nd^{\window}(4/m^{4/5})^{\window/3} \nonumber
	\end{align}
	Now doing a union bound over all sequences $s_i$,	
	\begin{align}
	P\Big[\absnorm{o_{s_i}-o_{s_j}} = 1 \; \forall s_i; s_j \in \mathcal{M}_{s_i}\Big] &\ge 1- n^2d^{2\window}(4/m^{4/5})^{\window/3}\nonumber\\
	&\ge 1- \frac{n^2m^{30\log_m n/16}4^{5\log_m n}}{m^{4\log_m n}}\nonumber\\
	&\ge 1- \frac{n^{5/\log_4 m}n^{31/8}}{n^4}\nonumber
	\end{align}
	which is $1-o(1)$. Hence every non-intersecting sequence of states in $\mathcal{M}$ has a different emission with high probability over the random assignment.
	
	%Consider any 2 hidden states $i$ and $j$. Let $P_i$ be the distribution over the $n$- length sequence of hidden states when a Markov chain $m_1$ starts at $i$, similarly let $P_j$ be the distribution over the $n$ length sequence of hidden states when a Markov chain $m_2$ starts at $j$. At each time step, every hidden state in the Markov chain either has a certain probability of being visited by $m_1$ and $m_2$. At each time step, label each hidden state as `+' if it has a higher probability of being visited by $m_1$ and as `-' if it has a higher probability of being visited by $m_2$. We do not label any states which have the same probability of being visited by $m_1$ or $m_2$. At each time step, we then label all transitions from each hidden state as `+' if the hidden state has a label `+' and `-' otherwise. Now consider all sequences which are always labeled as `+' and all sequences which are always as `-'. Note that these sequences are precisely the sequences where the chains $m_1$ and $m_2$ do not couple. Lets call the set of `+' sequences $\mathcal{S^{+}}$ and the set of `-' sequences $\mathcal{S^{-}}$. Note that at each time step $S^{+}$ and $S^{-}$ cannot share any hidden states because 
	
	Using this property of $O$, we will bound the condition number of $A$. We will lower bound $\sigma_{\min}^{(1)}(A)$. As $\sigma_{\min}^{(2)}(A) \ge\sigma_{\min}^{(1)}(A)/ \sqrt{n} $ and $\sigma_{\max}^{(2)}(A) \le \sqrt{n}$, $\kappa(A) \le n \sigma_{\min}^{(1)}(A)$. 
	
	Consider any $x\in\Real^n$ such that $\absnorm{x}=2$. We aim to show that $\absnorm{Ax}$ is large. Let $x^+$ be the vector of all positive entries of $x$ i.e. $x^+_i = \max(x_i,0)$ where $x_i$ denotes the $i$th entry of vector $x$. Similarly, $x^-$ is the vector of all negative entries of $x$, $x^-_i = \max(-x_i,0)$. We will find a lower bound for $\absnorm{Ax^+ -Ax^-}$. Note that because $A$ is a stochastic matrix, there exists and $x$ that minimizes $\absnorm{Ax}$ and has $1^Tx = 0$. Hence we will assume without loss of generality that $1^Tx = 0$, and hence $x^+$ and $x^-$ are valid probability distributions. Hence our goal is to show that for any two initial distributions $x^+$ and $x^-$ which have disjoint support,  $\absnorm{Ax^+ -Ax^-}\ge 1/\poly{n}$ which implies $\absnorm{Ax^+ -Ax^-}\ge 1/\poly{n}$ for any $x\in\Real^n$ such that $\absnorm{x}=2$. %, note that  We first argue that any $x$ which minimizes $\absnorm{Ax}$ should have $1^Tx=0$. Without loss of generality, assume $1^Tx^+ \ge 1^Tx^-$. Then we can write $\hat{x}^+=x^{}$.
	
	%Note that $\bar{x}^+=x^+/1^Tx^+$ and $\bar{x}^-=x^-/1^Tx^-$ define two initial distributions. 
	Note that $\absnorm{T^n x} >(\sigma_{\min}^{(1)}(T))^{\window}$. Hence the distributions $x^+$ and $x^-$ do not couple in $n$ time steps with probability at least $(\sigma_{\min}^{(1)}(T))^{\window}$. Note that $A{x}^+$ is a vector where the $i$th entry is the probability of observing string $a_i$ with the initial distribution ${x}^+$. Let $\mathcal{U}$ denote the set of all $n^{\window}$ sequences of hidden states over $\window$ time steps. We exclude all sequences which do not visit $(1-\alpha)\window$ hidden states in $\window$ time steps and sequences where at least one transition is outside the $(1-\delta)$ support of the current hidden state. Let $\mathcal{S}$ be the set of all sequences of hidden states which visit at least $(1-\alpha) n$ hidden states and where each transition is in the  $(1-\delta)$ support of the current hidden state. Let $\mathcal{X}=\mathcal{U}\backslash \mathcal{S}$. Note that for any distribution $p$, $Ap$ can be written as $Ap = \sum_{s\in\mathcal{X}}P(s|p) o_{s}$ where $P(s|p)$ is the probability of sequence $s$ with initial distribution $p$. Recall that $o_s \in \mathbb{R}^K$ is the vector of probabilities of outputs over the $K=m^{\window}$ size alphabet conditioned on the sequence of hidden states $s$. Taking $p$ to be $e_i$, each column $c_i$ of $A$ can be expressed as $c_i = \sum_{s\in\mathcal{X}}P(s|e_i) o_{s}$. Restricting to sequences in $\mathcal{S}$, we define two new matrices $A_{1}$ and $A_{2}$, with the $i$th column $c_{i,1}$ of $A_{1}$ defined as $c_{i,1} = \sum_{s\in\mathcal{S}}P(s|e_i) o_{s}$ and the $i$th column $c_{i,2}$ of $A_{2}$ is analogously defined as $c_{i,2} = \sum_{s\in\mathcal{X}}P(s|e_i) o_{s}$. Note that $A= A_{1}+ A_{2}$. Also, as every hidden state visits less than $(1-\alpha)\window$ hidden states over $\window$ time steps with probability at most $\delta$, and the probability of taking at least one transition outside the $(1-\delta)$ support is at most $\window \delta$, therefore $\sum_{s\in\mathcal{X}}P(s|e_i) \le \delta+ \window \delta$ for all $i$. Hence $\absnorm{A_{2}p} \le  \delta+ \window \delta$ for any vector $p$ with $\absnorm{p}=1$. 
	
	%We will now show that $\absnorm{A_1 x}\ge 1/k^{1.5} \; \forall x$, which implies that $\absnorm{Ax}\ge 0.5/k^{1.5}, \; \forall x$. 
	
	We will now lower bound $\absnorm{A_1 x}$. The high level proof idea is that if the two initial distributions do not couple then some sequences of states have more mass in one of the two distributions. Then, we use the fact that most sequences of states comprise of many distinct states to argue that two sequences of hidden states which do not intersect lead to very different output distributions. We combine these two observations to get the final result.
	
	Consider any $O$ which satisfies the property that every non-intersecting sequence of states has a different emission. We divide the output distribution $o_{s}$ of any sequence $s$ into two parts, $o_{s}^{(1)}$ and $o_{s}^{(2)}$. Define the $(1-\delta)$-support of $o_{s}$ as the set of possible outputs obtained when the emission at each time step belongs to the $(1-\delta)$ support of the output at that time step. We define $o_{s}^{(1)}$ as $o_{s}$ restricted to the $(1-\delta)$ support of $o_{s}$ and $o_{s}^{(2)}$ to be the residual vectors such that $o_{s} = o_{s}^{(1)} + o_{s}^{(2)}$. Note that $\absnorm{o_{s}^{(2)}}$ is at most $\window \delta$ for any sequence $s_i$. 
	
	Using our decomposition of the output distributions $o_{s}$ we will decompose $A_1$ as the sum of two matrices $A_1'$ and $A_1''$. The $i$th column $c_i'$ of $A_1'$ is defined as $c_i' = \sum_{s\in\mathcal{S}}P(e_i|s) o_{s}^{(1)}$. Similarly, the $i$th column $c_i''$ of $A_1''$ is defined as $c_i'' = \sum_{s\in\mathcal{S}}P(e_i|s) o_{s}^{(2)}$. As $\absnorm{o_{s_i}^{(2)}}\le \window \delta$ for every sequence $s_i$, $\absnorm{A_1''p}\le \window \delta$ for any vector $p$ with $\absnorm{p}=1$. %Hence it is sufficient to show that $\absnorm{A_1'x}\ge 1/k^{1.5}$ to prove that $\absnorm{A_1 x}\ge 1/k^{1.5} \; \forall x$.
	
	We will further divide every sequence $s$ into a set of augmented sequences $\{s_{a_1}, s_{a_2}, \dotsb, s_{a_K}\}$. Recall that $K=d^{\window}$ is the size of the output space in $\window$ time steps and $\{a_i, i \in [K]\}$ is the set of all possible output in $\window$ time steps. The probability of sequence $s_{a_i}$ is the product of the probability of sequence $s$ times the probability of the sequence $s$ emitting the observation $a_i$. Hence, the probability of each augmented sequence equals the product of the probability of making the corresponding transition at each time step and emitting the corresponding observation at that time step.
	
	For each output string $a_i$, there is a set of augmented sequences which have non-zero probability of emitting $a_i$. Consider the first string $a_1$. Let $\mathcal{S}_1^+$ be the set of all augmented sequences from the $x^+$ distribution with non-zero probability of emitting $a_1$, similarly let $\mathcal{S}_1^-$ be the set of all augmented sequences from the $x^-$ distribution with non-zero probability of emitting $a_1$. For any set of augmented sequences $\mathcal{S}$, let $|\mathcal{S}|$ denote the total probability mass of augmented sequences in $\mathcal{S}$. %Let $s=\{x_1, x_2,\dotsb, x_n\}$ be any augmented sequence of $n$ hidden states. 
	
%	\begin{lemma}
%		If $s^+\in \mathcal{S}_1^+$ and $s^- \in \mathcal{S}_1^-$, then $s^+$ and $s^-$ must meet at some state time step $t$. Moreover, if $t<n$ define $s_{+,-}=\{s_1^+, s_2^+, \dotsb, s_t^-, s_{t+1}^-, \dotsb, s_{n}^-\}$ and $s_{-,+}=\{s_1^-, s_2^-, \dotsb, s_t^+, s_{t+1}^+, \dotsb, s_{n}^+\}$. Then $s_{+,-} \in \mathcal{S}_1^+$ and $s_{-,+} \in \mathcal{S}_1^-$ .
%	\end{lemma}
%	\begin{proof}
%		The first statement follows from the constraint that sequences of hidden state which never meet must produce different outputs. The second statement from the definition of $\mathcal{S}_1^+$ and $\mathcal{S}_1^-$ and the definition of the sequences $s_{+,-}$ and $s_{-,+}$.
%	\end{proof}
	
	We now show that any assignment of augmented sequences to outputs $a_i$ induces a coupling for two Markov chains $m^+$ and $m^-$ starting with initial distributions $x^+$ and $x^-$ respectively and having transition matrix $T$. We denote two sequences $s^+$ and $s^-$ as having coupled if they meet at some time step $u$ and traverse the Markov chain together after $u$, and the probability of $s^+$ equals the probability of $s^-$. Let $\mathcal{C}$ denote some coupling, and $\bar{\mathcal{C}}$ denote the total probability mass on sequences which have not been coupled under $\mathcal{C}$. Note that the total variational distance between the distribution of hidden states at time step $n$ from the starting distribution $x^+$ and $x^-$ satisfies
	\begin{align}
	\absnorm{T^\window x^+-T^\window x^-}\le {\Big|\bar{\mathcal{C}}\Big|}\nonumber
	\end{align}
	for any coupling $\mathcal{C}$ with uncoupled mass $\bar{\mathcal{C}}$. This follows because all coupled sequences have the same distribution at time $\window$, hence the distance between the distributions is at most the mass on the uncoupled sequences.
	
	We claim that the sets of augmented sequences $\mathcal{S}_1^+$ and $\mathcal{S}_1^-$ can be coupled with residual mass ${|(A_{1}'x^+)_{1} -(A_{1}'x^-)_{1}|}$, where $(A_{1}'x^+)_{1}$ denotes the first entry of $A_{1}'x^+$. To verify this, first assume without loss of generality that $(A_{1}'x^+)_{1}>(A_{1}'x^-)_{1}$.  Let $P(a_1,h_i|x^+)$ be the probability of outputting $a_1$ in $\window$ time steps and being at hidden state $h_i$ at time 0, given the initial distribution $x^+$ at time 0. This is the sum of the probability of augmented sequences in $\mathcal{S}_1^+$ which start from hidden state $h_i$. Any coupling of the augmented sequences also induces a coupling of the probability masses $p^+=\{P(a_1,h_i|x^+), i \in [n]\}$ and $p^-=\{P(a_1,h_i|x^-), i \in [n]\}$. We will show that all of the probability mass $p^-$ can be coupled. Consider a simple greedy coupling scheme $\mathcal{C}_1$ which picks a starting state $i$ in $p^-$, traverses along the transitions from the state $i$ and couples as much probability mass on sequences starting from $i$ as possible whenever it meets a sequence from $p^+$, and repeats for all starting states, till there are no more sequences which can be coupled. We claim that the algorithm terminates when all of the probability mass in $p^-$ has been coupled. We prove by contradiction. Assume that there exists some probability mass $p^-$ which has not been coupled in the end. There must be also be some probability mass $p^+$ which has not been coupled. But all augmented sequences starting from hidden state $i$ meet with all sequences from hidden state $j$, so this means that more probability mass from $p^-$ can be coupled to $p^+$. This contradicts the assumption that there are no more augmented sequences which can be coupled. Hence all of the probability mass in $p^-$ has been coupled when the greedy algorithm terminates. Hence coupling $\mathcal{C}_1$ has residual mass $\Big|\bar{\mathcal{C}_1}\Big|$ at most ${|(A_{1}'x^+)_{1} -(A_{1}'x^-)_{1}|}$.
	
	Now, consider all outputs $a_i$ and couplings $\mathcal{C}_i$. Let $\mathcal{C}=\cup_i \mathcal{C}_i$. As our argument only couples the augmented sequences the mass $\absnorm{A_1''x^+}+ \absnorm{A_1''x^-}+\absnorm{A_2x^+}+\absnorm{A_2x^-}$ is never uncoupled. The total uncoupled mass is,
	\begin{align}
	\Big|\bar{\mathcal{C}}\Big| &= \sum_{i}^{}\Big|\bar{\mathcal{C}}\Big| + \absnorm{A_1''x^+}+ \absnorm{A_1''x^-}+\absnorm{A_2x^+}+\absnorm{A_2x^-}\nonumber\\
	\implies\Big|\bar{\mathcal{C}}\Big| &\le \absnorm{A_{1}'x^+ -A_{1}'x^-}+6\window\delta\nonumber\\
	\implies \absnorm{T^\window x^+-T^\window x^-}&\le \absnorm{A_{1}'x^+ -A_{1}'x^-}+6\window \delta\nonumber
	\end{align}
	Note that $\absnorm{T^\window x^+-T^\window x^-}\ge (\sigma_{\min}^{(1)}(T))^{\window} $. By condition 2 in Theorem \ref{thm:learnability}, $\sigma_{\min}^{(1)}(T)\ge 1/m^{c/20}$ therefore $\absnorm{T^\window x^+-T^\window x^-}\ge 1/n^{3c/4}$. Note that $\absnorm{Ax} \ge \absnorm{A_1'x}-\absnorm{A_1''x}-\absnorm{A_2 x}\ge 1/n^{3c/4}+10\window\delta$. As $\delta \le 1/n^c$, therefore $\absnorm{Ax}\ge 1/n^{3c/4}-0.5/n^{3c/4} \ge 0.5/n^{3c/4}$.
\end{proof}

We also mention the following corollary of Theorem \ref{thm:learnability}. Corollary \ref{thm:learnability_l2} is defined in terms of the minimum singular value of the matrix, $\sigma_{\min}^{(2)}(T)$, and is a slightly weaker but more interpretable version of Theorem \ref{thm:learnability}. The conditions are the same as in Theorem \ref{thm:learnability} with different bounds on $\delta_1, \delta_2, \delta_3$.% and follows by plugging in parameters and using the fact that $\sqrt{n}\sigma_{\min}^{(2)}(T)\le \sigma_{\min}^{(1)}(T) $
\begin{cor}\label{thm:learnability_l2}
	If an HMM satisfies $\delta_1,\delta_2,\delta_3\le 1/n^2$ and $\sigma_{\min}^{(2)}(T),\sigma_{\min}^{(2)}(T')\ge 1/m^{1/20}$ then with high probability over the choice of $O$, the parameters of the HMM learnable to within additive error $\epsilon$ with observations over windows of length $2\tau +1, \tau = 15\log_m n$ with the sample complexity being $\poly{n,1/\epsilon}$.
\end{cor}

On a side note, though $\sigma_{\min}^{(2)}(T)$ is much more easier to interpret than $\sigma_{\min}^{(1)}(T)$ -- for example, if the transition matrix is symmetric then the singular values are the same as the eigenvalues, and the eigenvalues of a matrix have well-known connections to the properties of the underlying graph, but, because $T$ is a stochastic matrix and all columns have unit $\ell_1$ norm, the $\ell_1$ norm seems better suited to measuring the gain of the matrix. For example, if the transition matrix has a single state which transitions to $d$ states with equal probability, then $\sigma_{\min}^{(2)}(T)\le 1/\sqrt{d}$ by choosing the vector which has unit mass on that state, hence if $d$ is large then $\sigma_{\min}^{(2)}(T)$ is always small even when the transition matrix is otherwise well-behaved. 

\subsection{Proof of Lemma \ref{lem:bound_dist}}\label{sec:lemma2}

\bounddist*
\begin{proof}
	The proof is in two parts. In the first part we show that $\absnorm{O_i-O_j}\ge 1/n^5$ with high probability. In the second part we show that ${\largenorm{{\frac{O_i}{\norm{O_i}}-\frac{O_j}{\norm{O_j}}}} \ge 1/n^{6.5}}$ if $\absnorm{O_i-O_j}\ge 1/n^5$.
	
	We will show that $\absnorm{O_i-O_j}\ge 1/n^5$ with high probability in the smoothed sense, which implies that it is also true in our model where they are chosen uniformly on a small support. Consider any two distributions $O_i$ and $O_j$. Let $O_i$ have largest mass on some state $f_i$ and next largest mass on another state $g_i$. Similarly, let $O_j$ have largest mass on some state $f_j$ and next largest mass on another state $g_j$. Let $x_1$ and $x_2$ be random variables uniformly distributed in $[0,1/n^2]$. Say we perturb $O_i$ by subtracting $x_1$ from the probability of $f_i$ and adding $x_1$ to the probability of $g_i$. Similarly, say we perturb $O_j$ by subtracting $f_2$ from the probability of $u_j$ and adding $x_2$ to the probability of $g_j$. With probability $1/n^3$ over the choice of $x_1$ and $x_2$, $|x_1-x_2|\ge 1/n^5$, which implies $\absnorm{O_i-O_j}\ge 1/n^5$. Therefore by a union bound over all pairs $O_i$ and $O_j$, $\absnorm{O_i-O_j}\ge 1/n^5$ with high probability. 
	
	We now show that ${\largenorm{{\frac{O_i}{\norm{O_i}}-\frac{O_j}{\norm{O_j}}}} \ge 1/n^{6.5}}$ when $\absnorm{O_i-O_j}\ge 1/n^5$. We prove the contrapositive via the following Lemma.
	
	\begin{lem}\label{lem:l1_l2}
		For any two vectors $v_1$ and $v_2$, ${\largeabsnorm{{\frac{v_1}{\absnorm{v_1}}-\frac{v_2}{\absnorm{v_2}}}} < 1/n^5}$ if ${\largenorm{{\frac{v_1}{\norm{v_1}}-\frac{v_2}{\norm{v_2}}}} \le 1/n^{6.5}}$.
	\end{lem}
	\begin{proof}
		As the claim is scale invariant, assume $\norm{v_1}=1$ and $\norm{v_2}=1$. As $\norm{v_1-v_2}\le 1/n^{6.5}$, therefore $\absnorm{v_1-v_2}\le 1/n^{6}$. Therefore $|\absnorm{v_1}-\absnorm{v_2}|\le 1/n^{6}$. Let $\absnorm{v_1}=x$, where $x\ge 1$, $\absnorm{v_2}=x+\delta$, where $|\delta|\le 1/n^{6}$. 
		\begin{align}
		\largenorm{{\frac{v_1}{\absnorm{v_1}}-\frac{v_2}{\absnorm{v_2}}}} &=
		\largenorm{{\frac{v_1}{x}-\frac{v_2}{x+\delta}}}\nonumber\\
		&= \frac{1}{x}\largenorm{{{v_1}-\frac{v_2}{1+\delta/x}}}\nonumber	\\
		&= \frac{1}{x}\norm{{{v_1}-{v_2}(1+\epsilon/x)}}\nonumber
		\end{align}
		for some $\epsilon$ with $|\epsilon| \le 2|\delta|$. Therefore using the triangle inequality,
		\begin{align}
		\largenorm{{\frac{v_1}{\absnorm{v_1}}-\frac{v_2}{\absnorm{v_2}}}} &\le 
		\frac{1}{x}\norm{{v_1}-{v_2}}+\frac{\epsilon}{x}\norm{v_2}\nonumber\\
		&\le 1/n^{6}+2/n^{6}< 1/n^{5.5}\nonumber\\
		\implies \largeabsnorm{{\frac{v_1}{\absnorm{v_1}}-\frac{v_2}{\absnorm{v_2}}}} &< 1/n^{5}\nonumber
		\end{align}
	\end{proof}
	Using Lemma \ref{lem:l1_l2}, it follows that ${\largenorm{{\frac{O_i}{\norm{O_i}}-\frac{O_j}{\norm{O_j}}}} > 1/n^{6.5}}$ when $\absnorm{O_i-O_j}\ge 1/n^5$
	%Recall that all hidden states have mass at most $\delta_3$ on all but $k$ states, with $k\le m^{1/3}$. For any distribution $p$, we define its $sup(p,1-\delta)$ as the set such that $p$ has mass at most $\delta$ outside that set. Define $p_i$ and $p_j$ as $O_i$ and $O_j$ restricted to the sets $sup(O_i,1-\delta_3)$ and $sup(O_j,1-\delta_3)$. We will show that $\absnorm{p_i-p_j}\ge $ with high probability. Note that $p_i$ and $p_j$ are randomly drawn from the simplex on their support. It is sufficient to consider the case when $p_i$ and $p_j$ have the same support.
	
	
\end{proof}

\subsection{Proof of Lemma \ref{determine}}\label{sec:lemma3}

\determine*
	\begin{proof}
		For the output distributions corresponding to sequence $s_i$ and $s_j$ to not have disjoint supports, the hidden state visited by the two sequences at every time step must have overlapping output distributions. The probability of any pair of hidden states having overlapping support is at most $1-(1-2k/m)^k\le 4k^2/m$. 
		
		Consider the graph $G$ on $n$ nodes, where we connect node $u$ and node $v$ if sequence $s_i$ and $s_j$ are simultaneously at hidden states $v$ and $v$ at some time step. As each sequence visits at least $(1-\alpha)\window$ different hidden states, at least $(1-\alpha)\window$ nodes in $G$ have non-zero degree. Consider any connected component $C$ of the graph with $p$ nodes. Note that the probability of the output distributions corresponding to each edge in the connected component $C$ to be overlapping equals the probability of the output distributions of each node in $C$ to be overlapping. This is at most $\Big(\frac{4k^2}{m}\Big)^{p-1}$. Now, let there be $M$ connected components in  graph each of which has $p_i$ nodes. The probability of the sequences having the same support is at most
		\begin{align}
		P\Big[\absnorm{o_{s_i}-o_{s_j}} < 1\Big]&\le \Pi_{i=1}^M \Big(\frac{4k^2}{m}\Big)^{p_i-1}\nonumber\\
		&\le \Big(\frac{4k^2}{m}\Big)^{\sum_{i}^{}(p_i-1)} 
		\le \Big(\frac{4k^2}{m}\Big)^{(1-\alpha) \window - M} \nonumber\\
		&\le \Big(\frac{4k^2}{m}\Big)^{(1-\alpha) \window/2}\nonumber
		\end{align}
		where the last step follows because $\sum_{i}^{}p_i$ is the number of nodes which have non-zero degree, which is at least $ \ge (1-\alpha)t$, and as every connected component has at least 2 nodes, there are at most $(1-\alpha)t/2$ connected components, therefore $M\le (1-\alpha)t/2$.
	\end{proof} 

%\undirectgirth*
%\begin{proof}
%At each time step, the random walk can either visit a new node or go back to a previously visited node. As the girth of the graph $g>\tau$, therefore the only way the random walk can go back to a previously visited node is if it goes back to the node it came from in the previous time step. The probability of this is at most $1/d$ as all nodes in the graph have degree $d$. 
%
%Let $X_i$ be the random variable denoting whether the random walk visits a new node in the $i$th time step. Note that $P(X_i=1)\ge 3/4$. Also, the random variables  
%\end{proof}

==> NIPS Arxiv/long_term_mixing.tex <==
\vspace{-12pt}
\section{Discussion on long-term dependencies in HMMs}\label{sec:long_term}
\vspace{-8pt}
In this section, we discuss long-term dependencies in HMMs, and show how our results on overcomplete HMMs improve the understanding of how HMMs can capture long-term dependencies, both with respect to the Markov chain and the outputs. Recall the definition of $\sigma_{\min}^{(1)}(T)$:
\vspace{-5pt}
\begin{align}
\sigma_{\min}^{(1)}(T) = \min_{x\in \mathbb{R}^n}\frac{\absnorm{Tx}}{\absnorm{x}}\nonumber
\end{align}
%In this short section, we discuss why $\sigma_{\min}^{(1)}(T)$ is a natural parameter to measure the long-term dependence in the transition matrix. 
We claim that if $\sigma_{\min}^{(1)}(T)$ is large, then the transition matrix preserves significant information about the distribution of hidden states at time 0 at a future time $t$, for all initial distributions at time 0. Consider any two distributions $p_0$ and $q_0$ at time 0. Let $p_t$ and $q_t$ be the distributions of the hidden states at time $t$ given that the distribution at time 0 is $p_0$ and $q_0$ respectively. Then the $\ell_1$ distance between $p_t$ and $q_t$ is $\absnorm{p_t-q_t}\ge (\sigma_{\min}^{(1)}(T))^t \absnorm{p_0-q_0}$, verifying our claim. It is interesting to compare this notion with the mixing time of the transition matrix. Defining mixing time as the time until the $\ell_1$ distance between any two starting distributions is at most $1/2$, it follows that the mixing time $\tau_{\text{mix}}\ge 1/\log (1/\sigma_{\min}^{(1)}(T))$, therefore if $\sigma_{\min}^{(1)}(T))$ is large then the chain is slowly mixing. However, the converse is not true---$\sigma_{\min}^{(1)}(T)$ might be small even if the chain never mixes, for example if the graph is disconnected but the connected components mix very quickly. Therefore, $\sigma_{\min}^{(1)}(T)$ is possibly a better notion of the long-term dependence of the transition matrix, as it requires that information is preserved about the past state ``in all directions''.

Another reasonable notion of the long-term dependence of the HMM is the long-term dependence in the output process instead of in the hidden Markov chain, which is the utility of past observations when making predictions about the distant future (given outputs $y_{-\infty},\dots,y_1, y_2, \dots, y_t$, at time $t$ how far back do we need to remember about the past to make a good prediction about $y_t$?). This does not depend in a simple way on the $T$ and $O$ matrices, but we do note that if the Markov chain is fast mixing then the output process can certainly not have long-term dependencies. We also note that with respect to long-term dependencies in the output process, the setting $m\ll n$ seems to be much more interesting than when $m$ is comparable to $n$. The reason is that in the small output alphabet setting we only receive a small amount of information about the true hidden state at each step, and hence longer windows are necessary to infer the hidden state and make a good prediction. 
We also refer the reader to \citet{kakade2016prediction} for related discussions on the memory of output processes of HMMs.
%If the size of the output alphabet is instead comparable to the number of hidden states, then the outputs may provide a lot of information about the current hidden state at each time step. In this case, short windows may be sufficient for correctly guessing the hidden state and hence predicting the next output to a high accuracy. 

\begin{comment}

In this short section, we discuss long-term dependencies in HMMs with respect to both the Markov chain and the output process. Recall the definition of $\sigma_{\min}^{(1)}(T)$--
\begin{align}
\sigma_{\min}^{(1)}(T) = \min_{x\in \mathbb{R}^n}\frac{\absnorm{Tx}}{\absnorm{x}}\nonumber
\end{align}

We claim that $\sigma_{\min}^{(1)}(T)$ is a natural parameter to measure the long-term dependence in the transition matrix. If $\sigma_{\min}^{(1)}(T)$ is large then the transition matrix preserves significant information about the distribution of hidden states at time 0 at a future time $t$, for all initial distributions at time 0. Consider any two distributions $p_0$ and $q_0$ at time 0. Let $p_t$ and $q_t$ be the distributions of the hidden states at time $t$ given that the distribution at time 0 is $p_0$ and $q_0$ respectively. Then the $\ell_1$ distance between $p_t$ and $q_t$ is $\absnorm{p_t-q_t}\ge (\sigma_{\min}^{(1)}(T))^t \absnorm{p_0-q_0}$.

It is interesting to compare this notion with the mixing time of the transition matrix. Defining mixing time as the time until the $\ell_1$ distance between any two starting distributions is at most $1/2$, it follows that the mixing time $\tau_{\text{mix}}\le 1/\log (1/\sigma_{\min}^{(1)}(T))$. However, the converse is not true, $\sigma_{\min}^{(1)}(T)$ might be small even if the chain never mixes, for example if the graph is disconnected but the connected components mix very quickly. Therefore, $\sigma_{\min}^{(1)}(T)$ is possibly a better notion of the long-term dependence of the transition matrix, as it requires the transition matrix to preserve the information about the past state ``in all directions''.

Another very reasonable notion of the long-term dependence of the HMM is the long-term dependence in the output process instead of in the Markov chain, which is the utility of past observations when making predictions about the distant future. This does not depend in a simple way on the $T$ and $O$ matrices, but we do note that if the Markov chain is fast mixing then the output process can certainly not have long-term dependencies. As pointed out in the introduction,  with respect to long-term dependencies in the output process, the setting $m\ll n$ seems to be much more interesting than when $m$ is comparable to $n$ as it limits how much information we obtain about the underlying Markov chain at each step. We also refer the reader to \cite{kakade2016prediction} for related discussions on the memory of output processes of HMMs.

\end{comment}

%On a side note, though $\sigma_{\min}^{(2)}(T)$ is much more easier to interpret than $\sigma_{\min}^{(1)}(T)$ -- for example, if the transition matrix is symmetric the singular values are the same as the eigenvalues, and the eigenvalues of a matrix have well-known connections to the properties of the underlying graph, but, because $T$ is a stochastic matrix and all columns have unit $\ell_1$ norm, the $\ell_1$ norm is better suited to measuring the gain of the matrix.\footnote{For example, if the transition matrix has a  state which transitions to $d$ states with equal probability, then  $\sigma_{\min}^{(2)}(T)\le 1/\sqrt{d}$ by choosing $x$ to have unit mass on that state, hence if $d$ is large $\sigma_{\min}^{(2)}(T)$ is always small even when the transition matrix is otherwise well-behaved.} %We obtain tighter results using $\sigma_{\min}^{(1)}(T)$, and these naturally imply slightly weaker results for $\sigma_{\min}^{(2)}(T)$


==> NIPS Arxiv/lower_bound.tex <==
\section{Lower bounds for learning dense, random HMMs}\label{sec:lower_bound}

In this section, we state our lower bound that it is not possible to efficiently learn HMMs where the underlying transition matrix is a random walk on a graph with a large degree and $m$ is small with respect to $n$. We actually show a stronger result than this -- we show that the number of bits of information contained in polynomial number of samples from such an HMM is a negligible fraction of the total number of bits of information needed to specify the transition matrix in these cases, showing that approximate learning is also information theoretically impossible.
\begin{restatable}{thm2}{lowerbound}\label{thm:lower_bound}
	Consider the class of HMMs with $n$ hidden states and $m$ outputs and $m=\polylog{n}$ with the transition matrix chosen to be a $d$-regular graph, with $d=n^\epsilon$ for some $\epsilon>0$. Then at least $\Omega(nd)$ bits of information are needed to specify the choice of the transition matrix. However, if the observation matrix $O$ is randomly chosen such that the columns of $O$ are chosen independently and $\E[O_{ij}]=1/m$ for all $i,j$, then the number of bits of information contained in polynomially many samples over a window of length $N=\poly{n}$ is at most $\tilde{\mathcal{O}}(n)$, with high probability over the choice of $O$, where the $\tilde{\mathcal{O}}$ notation hides polylogarithmic factors in $n$.
\end{restatable}
\noindent \emph{Proof sketch.}
The proof consists of two steps--in the first step we show that the information contained in polynomially many observations over windows of length $\tau=\lfloor \log_m n \rfloor$ is not sufficient to learn the HMM. The proof of this part relies on a counting argument and a lower bound on the number of random regular graphs with a given degree. We then show that the information contained in polynomial samples over longer windows is not much larger than the information contained in polynomial samples over a window length of $\tau$. This is the main technical part, and we need to show that the hidden state at time 0 does not have much influence on the hidden state at time $t$, conditioned on the outputs from time 0 to $t$. The conditioning makes this tricky, as the probabilities of the hidden states no longer evolve under the transition matrix of the Markov chain. We get around this by showing that the probability of the hidden states after conditioning on the observations evolves under a time-inhomogeneous Markov chain, and the transition matrices at every time step are related to the outputs from time 1 to $t$ and the original transition matrix. We analyze the spectrum of the time-inhomogeneous transition matrices to show that the influence of the hidden state at time 0 decays at every step and is small at time $t$. \hfill $\square$

We would like to point out that our techniques to prove the information theoretic lower bound appear to be generally useful for analyzing the influence of the hidden state at time 0 on the hidden state at time $t$, conditioned on the outputs from time 0 to $t$, This is a measure of how much value there is to observations before time 0 for predicting the observation at time $t+1$, conditioned on the intermediate observations from time 0 to $t$. This is a natural notion of the memory of the output process.

==> NIPS Arxiv/lower_bound_proof.tex <==
\section{Proof of lower bound for dense HMMs}\label{sec:lower_bound_proof}

%In this section, we prove our lower bound that it is not possible to efficiently learn HMMs where the underlying transition matrix is a random walk on a graph with a large degree and $m$ is small with respect to $n$. We actually show a stronger result than this -- we show that the number of bits of information contained in polynomial number of samples from such an HMM is a negligible fraction of the total number of bits of information needed to specify the transition matrix in these cases, showing that approximate learning is also information theoretically impossible. We provide a proof sketch followed by the formal proof.

%\begin{restatable}{thm}{lowerbound}\label{thm:lower_bound}
%	Consider the class of HMMs with $n$ hidden states and $m$ outputs and $m=\polylog{n}$ with the transition matrix chosen to be a $d$-regular graph, with $d=n^\epsilon$ for some $\epsilon>0$. Then at least $\Omega(nd)$ bits of information are needed to specify the choice of the transition matrix. However, if the observation matrix $O$ is randomly chosen such that the columns of $O$ are chosen independently and $\E[O_{ij}]=1/m$ for all $i,j$, then the number of bits of information contained in polynomially many samples over a window of length $N=\poly{n}$ is at most $\tilde{\mathcal{O}}(n)$, with high probability over the choice of $O$, where the $\tilde{\mathcal{O}}$ notation hides polylogarithmic factors in $n$.
%\end{restatable}
\begin{thm2}
	Consider the class of HMMs with $n$ hidden states and $m$ outputs and $m=\polylog{n}$ with the transition matrix chosen to be a $d$-regular graph, with $d=n^\epsilon$ for some $\epsilon>0$. Then at least $\Omega(nd)$ bits of information are needed to specify the choice of the transition matrix. However, if the observation matrix $O$ is randomly chosen such that the columns of $O$ are chosen independently and $\E[O_{ij}]=1/m$ for all $i,j$, then the number of bits of information contained in polynomially many samples over a window of length $N=\poly{n}$ is at most $\tilde{\mathcal{O}}(n)$, with high probability over the choice of $O$, where the $\tilde{\mathcal{O}}$ notation hides polylogarithmic factors in $n$.
\end{thm2}
\begin{proof}
	By \citet{shamir1984large} (also see \citet{krivelevich2001random}), the number of $d$-regular graphs on $n$ vertices is at least ${\dbinom{\binom{n}{2}}{ nd/2}}\exp(-nd^{0.5+\delta})$ for any fixed $\delta>0$. This can be bounded from below as follows---
	\begin{align}
	{\dbinom{\binom{n}{2}}{ nd/2}}\exp(-nd^{0.5+\delta})&=\Big(\frac{n-1}{d}\Big)^{nd/2}\exp(-nd^{0.5+\delta})\nonumber\\
	&\ge 2^{nd/2-nd^{0.5+\delta}}\nonumber
	\end{align}
	Hence the number of bits needed to specify a randomly chosen $d$-regular graph on $n$ vertices is at least $\Omega(nd)$. 
	
	Note that if we only get observations over a window of length $\tau = \lfloor \log_m n \rfloor$, and we obtain $\poly{n}$ samples, then the total information in those samples is at most $\tilde{O}(n)$, where the $\tilde{O}$ hides polylogarithmic factors in $n$. This is because there are at most $m^{\tau} \le n$ possible outputs, each of which can take $\poly{n}$ different values as there are $\poly{n}$ samples. We will now show that getting polynomially many samples over windows of length $N=\poly{n}$ is equivalent to getting polynomially many samples over windows of length $\tau$.
	
	For notational convenience, we will refer to $P[o_t=i]$, the probability of the output at time $t$ being $i$, as $P[o_t]$ whenever the assignment to the random variable is clear from the context. The probability of any sequence of outputs $\{o_1,o_2,\dotsb, o_{N}\}$ can be written down as follows using chain rule,
	\begin{align}
	P[o_1,o_2,\dotsb, o_N] &= P[o_1]P[o_2|o_1]P[o_3|o_1,o_2]\dotsb P[o_N|o_{1},\dotsb,o_{N-1}]\nonumber\\
	&=\Pi_{t=1}^N P[o_t|o_1, \dotsb, o_{t-1}]\nonumber
	\end{align}
	In order to prove that the probabilities of sequences of length $N$ can be well-approximated using sequences of length $\tau$, for $t>\tau$, we will approximate the probability $P[o_t|o_{1},\dotsb,o_{t-1}]$ by $P[o_t|o_{t-\tau+1},\dotsb,o_{t-1}]$. Hence our estimate of the probability of sequence $\{o_1,o_2,\dotsb, o_N\}$ is
	\begin{align}
	\hat{P}[\{o_1,o_2,\dotsb, o_N\}] &= \Pi_{t=1}^\tau {P}[o_t|o_{(t-\tau+1)\vee 1}, \dotsb, o_{t-1}]\nonumber
	\end{align}
	where $a\vee b$ denotes $\max(a,b)$. If 
	\begin{align}
	\absnorm{P[o_t|o_1, \dotsb, o_{t-1}]-{P}[o_t| o_{(t-\tau+1)\vee 1}, \dotsb,o_{t-1}]} \le \epsilon \label{eq:est_short}
	\end{align}
	for all $t\le N$ and assignments to $\{o_1, \dotsb, o_{t}\}$, then
	\begin{align}
	\Big|P[o_1,o_2,\dotsb, o_N]-\hat{P}[o_1,o_2,\dotsb, o_N] \Big| \le O(\epsilon N )\nonumber
	\end{align}
	for all assignments to $\{o_1, \dotsb, o_{N}\}$. Hence the probabilities of windows of length $N$ can be estimated from windows of length $\tau$ up to an additive error of $O(\epsilon N )$. Therefore, if we can show that $\epsilon \le o(1/\poly{n})$, then given the true probabilities of windows of length $\tau$, it is possible to estimate the true probabilities over windows of length $N=\poly{n}$ up to an inverse super-polynomial factor of $n$. Given empirical probabilities of windows of length $\tau$ up to an accuracy of $\delta$, it is possible to estimate the true probabilities over windows of length $N$ up to an error of $(\epsilon + \delta)N$. As $\epsilon N$ is inverse super-polynomial in $N$, getting $S$ samples over windows of length $N$ is equivalent to getting $\poly{N,S}$ samples over windows of length $\tau$. Therefore, the information contained in polynomially many samples over windows of length $N$ is entirely contained in the polynomially many samples over windows of length $\tau$ (the polynomials would be different, but this does not concern us as we have shown that the information in polynomially many samples over windows of length $\tau$ is always $\tilde{O}(n)$). Hence the information contained in polynomially many samples over windows of length $N$ can be at most $\tilde{O}(n)$. 
	
	We will now prove Eq. \ref{eq:est_short}. First, note that Eq. \ref{eq:est_short} can be written in terms of the probabilities of the hidden states as follows,
	\begin{align}
	P[o_t=j|o_1, \dotsb, o_{t}] = \sum_{i=1}^{n}P[o_t=j|h_t=i]P[h_t=i|o_1, \dotsb, o_{t}]\nonumber
	\end{align}
	Therefore, it is sufficient to show the following, which says that the distribution of the hidden states conditioned on the two observation windows is similar--
	\begin{align}
	\absnorm{P[h_{t}|o_1, \dotsb, o_{t-1}]-{P}[h_t| o_{(t-\tau+1)\vee 1}, \dotsb,o_{t-1}]} \le \epsilon \label{eq:rtp1}
	\end{align}
	for all $t\le N$ and assignments to $\{o_1, \dotsb, o_{t-1}\}$. Note that we do not need to worry about the case when $t\ge \tau$ as the observation windows under consideration are the same for both terms. We will shift our windows and fix $t=\tau$ to make notation easy, as the process is stationary this can be done without loss of generality. Hence we will rewrite Eq. \ref{eq:rtp1} as follows, ignoring the cases when the terms are the same because $(t-\tau+1)\vee 1=1$. 
	\begin{align}
	\Big|P[h_{\tau}|o_1, \dotsb, o_{\tau-1}]-{P}[h_{\tau}|o_{z}, \dotsb, o_{\tau-1}]\Big| \le \epsilon \nonumber
	\end{align}
	for all $z \in[\tau-N+1,0]$. %$P[h_{\tau}|o_1, \dotsb, o_{\tau-1}]$ and ${P}[h_{\tau}|o_{z}, \dotsb, o_{(\tau-1)}]$ can be rewritten as,
	%\begin{align}
	%P[h_{\tau}|o_1, \dotsb, o_{\tau-1}] &= \sum_{i=1}^{n}P[h_0=i|o_1, \dotsb, o_{\tau-1}] P[h_{\tau}|h_0=i,o_1, \dotsb, o_{\tau-1}] \nonumber\\
	%{P}[h_\tau|o_{z}, \dotsb, o_{\tau-1}] &= \sum_{i=1}^{n}P[h_0=i|o_{z}, \dotsb, o_{\tau-1}] P[h_{\tau}|h_0=i,o_1, \dotsb, o_{\tau-1}]\nonumber
	%\end{align}
	%where we could simplify $P[h_{\tau}|h_0=i,o_z, \dotsb, o_{\tau-1}]=P[h_{\tau}|h_0=i,o_1, \dotsb, o_{\tau-1}]$ as conditioned on the hidden state at time 0, the observations before time 0 do not affect the distribution of future hidden states. Let the distribution $P[h_0=i|o_1, \dotsb, o_{\tau-1}]$ be $p_1$ and the distribution $P[h_0=i|o_{z}, \dotsb, o_{\tau-1}]$ be $p_2$. We will now analyze the common $P[h_{\tau}|h_0=i,o_1, \dotsb, o_{\tau-1}]$ term. Note that if there was no conditioning on the observations but only on the hidden state, then it would be easy to directly write down the conditional probabilities using the transition matrix of the HMM. Though the transition matrix $T$ cannot be used in this case, we can use something just as good for our purpose.
	
	Define the modified transition matrix $T^{(t)}$ as ${T^{(t)}_{i,j}=P[h_{t+1}=j|h_t=i,o_{t+1},\dotsb,o_{\tau-1}]}$. For any $s \in [0,\tau]$, we claim that,
	\begin{align}
	P[h_{s}|o_z, \dotsb, o_{\tau- 1}]=\Big(\Pi_{t=1}^{s} T^{(t)}\Big)P[h_0|o_z, \dotsb, o_{\tau- 1}]\nonumber
	\end{align}
	for all $z \in[\tau-N+1,0]$. Therefore $T^{(t)}$ serves the role of the transition matrix at time $t$ in our setup. The proof of this follows from a simple induction argument on $s$. The base case $s=0$ is clearly correct. Let the statement be true up to some time $p$. Then we can write,
	\begin{align}
	P[h_{p+1}|o_z, \dotsb, o_{\tau-1}]&=\sum_{i}^{}P[h_p=i,h_{p+1}|o_z, \dotsb, o_{\tau-1}]\nonumber\\
	&=\sum_{i}^{}P[h_p=i|o_z, \dotsb, o_{\tau-1}]P[h_{p+1}|h_p=i,o_z, \dotsb, o_{\tau}]\nonumber\\
	%	&=\sum_{i}^{}P[h_p=i|o_1, \dotsb, o_{(i-1)\vee 1}]P[h_{p+1}=i|h_p=i,o_1, \dotsb, o_{(i-1)\vee 1}]\\
	&=\sum_{i}^{}P[h_{p+1}|h_p=i,o_{p+1}, \dotsb,o_{\tau-1}]\Big(\Pi_{t=1}^{p} T^{(t)}\Big)P[h_0|o_z, \dotsb, o_{\tau- 1}]\nonumber \\	
	&=\Big(\Pi_{t=1}^{p+1} T^{(t)}\Big)P[h_0|o_z, \dotsb, o_{\tau- 1}]\nonumber
	\end{align}
	where we could simplify $P[h_{p+1}|h_p=i,o_z, \dotsb, o_{\tau-1}]=P[h_{p+1}|h_p=i,o_{p+1}, \dotsb, o_{\tau-1}]$ as conditioned on the hidden state at time $p$, the observations at and before time $p$ do not affect the distribution of future hidden states. Therefore, our task now reduces to analyzing the spectrum of the time-inhomogeneous transition matrices $T^{(t)}$. The following Lemma does this.
	\begin{restatable}{lem}{boundspectrum}\label{lem:bound_spectrum}
		For any $x$ with $\norm{x}=1$ and $1^Tx=0$, $\norm{T^{(t)}x}\le \alpha+\lambda$ where $\alpha \le \sqrt{\frac{100m^3\log^3 n}{2d}}$  and $\lambda <3/\sqrt{d}$. Therefore if $d=n^{\epsilon}$ for some $\epsilon>0$ and $m=\polylog{n}$, then $\norm{T^{(t)}x}\le n^{-\epsilon_1}$ for some $\epsilon_1>0$. 
	\end{restatable}
	Given Lemma \ref{lem:bound_spectrum}, we will show $\epsilon=o(1/\poly{n})$. Let $p_1 = P[h_0|o_1, \dotsb, o_{\tau- 1}]$ and $p_2 = P[h_0|o_z, \dotsb, o_{\tau- 1}]$ for any $z<1$. We can write,
	\begin{align}
	 P[h_0|o_1, \dotsb, o_{\tau- 1}] - P[h_0|o_z, \dotsb, o_{\tau- 1}]  = \Big(\Pi_{t=1}^{\tau} T^{(t)}\Big)(p_1-p_2)\nonumber
	\end{align}
	Let $p_1-p_2 = x$. Note that $\norm{x}\le 1$ and $1^Tx =0$. Furthermore, as $T^{(t)}$ is stochastic for every $t$, therefore $1^T \Big(\Pi_{t=1}^{s} T^{(t)}\Big)x$ is also $0$ for every $s$. Hence we can use Lemma \ref{lem:bound_spectrum} to say,
	\begin{align}
	\norm{P[h_0|o_1, \dotsb, o_{\tau- 1}] - P[h_0|o_t, \dotsb, o_{\tau- 1}]}&\le (2(\alpha+\lambda))^{\tau}\nonumber\\
	\implies \absnorm{P[h_0|o_1, \dotsb, o_{\tau- 1}] - P[h_0|o_t, \dotsb, o_{\tau- 1}]}&\le \sqrt{n}(\alpha+\lambda)^{\tau}\nonumber\\
	&\le n^{- \log^{\delta} n}\nonumber
	\end{align}
	for a fixed $\delta>0$. This is superpolynomial in $n$, proving Theorem \ref{thm:lower_bound}. We will now prove Lemma \ref{lem:bound_spectrum}. 
	\boundspectrum*
	\begin{proof}
		We show that $T^{(t)}$ has a simple decomposition, $T^{(t)}=O^{(t)}TE^{(t)}$, where $O^{(t)}$ is a diagonal matrix with $O^{(t)}_{i,i}=P(o_t,\dotsb,o_{\tau}|h_t=i)$ and $E^{(t)}$ is another diagonal matrix with $E^{(t)}_{i,i}= P[o_{t+1},\dotsb,o_{\tau}|h_{t}=i]$. This is because,
		\begin{align}
		P[h_{t+1}=j|h_t=i,o_{t+1},\dotsb,o_{\tau}] &= \frac{P[h_{t+1}=j|h_t = i]P[o_{t+1},\dotsb,o_{\tau}|h_{t+1}=j]}{\sum_{j}^{}P[h_{t+1}=j|h_t = i]P[o_{t+1},\dotsb,o_{\tau}|h_{t+1}=j]}\nonumber\\
		&= \frac{P[h_{t+1}=j|h_t = i]P[o_{t+1},\dotsb,o_{\tau}|h_{t+1}=j]}{P[o_{t+1},\dotsb,o_{\tau}|h_{t}=i]}\nonumber
		\end{align}
		As $T$ is the normalized adjacency of a $d-$regular graph, the eigenvector corresponding to the eigenvalue 1 is the all ones vector, and all subsequent eigenvectors are orthogonal to the all ones vector. Also, the second eigenvalue and all subsequent eigenvalues of $T$ are at most $3/\sqrt{d}$, due to \citet{friedman2003proof}. 
		
		To analyze $O^{(t)}$ and $E^{(t)}$, we need to first derive some properties of the randomly chosen observation matrix $O$. We claim that,
		\begin{lem}\label{lem:bound_O}
			Denote $x_{ij}$ to be the random variable denoting the probability of hidden state $i$ emitting output $j$. If $\{x_{ij},i \in [n]\}$ are independent and $\E[x_{ij}]=1/m$ for all $i$ and $j$, then for all outputs $j \in [m]$ and hidden states $i\in [n]$, ${\Big|P[o_{t+1}=j|h_t=i]-1/m\Big|\le \sqrt{6\log n/(dm)}}$.
		\end{lem}
		\begin{proof}
			The result is a simple application of Chernoff bound and a union bound. Without loss of generality, let the set of neighbors of hidden state $i$ be the hidden states $\{1,2,\dotsb,d\}$. ${P[o_{t+1}=j|h_t=i]}$ is given by,
			\begin{align}
			P[o_{t+1}=j|h_t=i] = (1/d)\sum_{k=1}^{d}x_{kj}\nonumber
			\end{align}
			Let $X_{ij}=\sum_{k=1}^{d}x_{kj}$. Note that the $x_{kj}$'s are all independent and bounded in the interval $[0,1]$ with $\E[x_{kj}]=1/m$. Therefore we can apply Chernoff bound to show that,
			\begin{align}
			P\Big[|X_{ij}-d/m|&\ge \sqrt{\frac{6d\log n}{m}}\Big]\le 2\exp(-2\log n)\le 2/n^2\nonumber
			\end{align}
			Therefore, ${\Big|P[o_{t+1}=j|h_t=i]-1/m\Big|\le \sqrt{6\log n/(dm)}}$ with failure probability at most $1/n^2$. Hence by performing a union bound over all hidden states and outputs, with high probability $|P[o_{t+1}=j|h_t=i]-1/m|\le \sqrt{6\log n/(dm)}$ for all all outputs $j \in [m]$ and hidden states $i\in [n]$.
		\end{proof}
		Using Lemma \ref{lem:bound_O}, it follows that 
		$$P[o_{t+1},\dotsb,o_{\tau}|h_t=i] \in \Big[\frac{1}{m^{\tau-t}}\Big(1-\sqrt{\frac{3m\log^3 n}{2d}}\Big),\frac{1}{m^{\tau-t}}\Big(1+\sqrt{\frac{24m\log^3 n}{d}}\Big)\Big]$$ This is because using Lemma \ref{lem:bound_O}, conditioned on any hidden state at any time $t$, $${P[o_{t+1}=j|h_t=i]} \in {\Big[\Big(\frac{1}{m}-\sqrt{\frac{6\log n}{dm}}\Big),\Big(\frac{1}{m}+\sqrt{\frac{6\log n}{md}}\Big)\Big]}$$ for all outputs $j$, hidden states $i$  and $t\in[0,\tau]$ hence the probability of emitting the sequence of outputs $\{o_t,\dotsb,o_{\tau}\}$ starting from any hidden state is at most $$ \Big(\frac{1}{m}+\sqrt{\frac{6\log n}{md}}\Big)^{\tau-t}\le \frac{1}{m^{\tau-t}}\Big(1+\sqrt{\frac{24m\tau^2\log n}{d}}\Big)\le \frac{1}{m^{\tau-t}}\Big(1+\sqrt{\frac{24m\log^3 n}{d}}\Big)$$ and similarly for the lower bound. Therefore $O^{(t)}_{i,i}=P[o_{t+1},\dotsb,o_{\tau}|h_{t+1}=i]$ can be bounded as follows
		\begin{align}
		P[o_{t+1},\dotsb,o_{\tau}|h_{t+1}=i] &=P[o_{t+1}|h_{t+1}=i]P[o_{t+2},\dotsb,o_{\tau}|h_{t+1}=i]\le P[o_{t+2},\dotsb,o_{\tau}|h_{t+1}=i]\nonumber\\
		\implies O^{(t)}_{i,i} &\le \frac{1}{m^{\tau-t-1}}\Big(1+\sqrt{\frac{24m\log^3 n}{d}}\Big)\; \forall i,t\nonumber
		\end{align}
		We will now bound the entries of $\tilde{E}^{(t)}$. Note that
		\begin{align}
		1/E^{(t)}_{i,i}&= P[o_{t+1},\dotsb,o_{\tau}|h_{t}=i]\nonumber\\
		\implies & \frac{1}{m^{\tau-t}}\Big(1-\sqrt{\frac{3m\log^3 n}{2d}}\Big)\le 1/E^{(t)}_{i,i}\le \frac{1}{m^{\tau-t}}\Big(1+\sqrt{\frac{24m\log^3 n}{d}}\Big)  \nonumber\\
		\implies& m^{\tau-t}\Big(1-\sqrt{\frac{24m\log^3 n}{2d}}\Big)\le E^{(t)}_{i,i}\le m^{\tau-t}\Big(1+\sqrt{\frac{12m\log^3 n}{d}}\Big)  \nonumber
		\end{align}
		
		
%		\begin{align}
%		1/E^{(t)}_{i,i}&=\sum_{j=1}^{n}T_{ji}P[o_{t+1},\dotsb,o_{\tau}|h_{t+1}=j]=
%		\sum_{j\in N(i)}^{n}(1/d)P[o_{t+1}|h_{t+1}=j]P[o_{t+2},\dotsb,o_{\tau}|h_{t+1}=j]\nonumber\\
%		&= X_{h_t=i, o_t=j}P[o_{t+2},\dotsb,o_{\tau}|h_{t+1}=j]\nonumber\\
%		\implies& \frac{1}{m^{\tau+1}}\Big(1-\sqrt{\frac{3m\log^3 n}{2d}}\Big)\le 1/E^{(t)}_{i,i}\le \frac{1}{m^{\tau+1}}\Big(1+\sqrt{\frac{24m\log^3 n}{d}}\Big)  \nonumber\\
%		\implies& m^{\tau+1}\Big(1-\sqrt{\frac{24m\log^3 n}{2d}}\Big)\le E^{(t)}_{i,i}\le m^{\tau+1}\Big(1+\sqrt{\frac{12m\log^3 n}{d}}\Big)  \nonumber\nonumber
%		\end{align}
		
		We can cancel the factor of $m^{\tau-t-1}$ appearing in the numerator of the upper bound for $E_{ii}^{(t)}$ and denominator of the upper bound for $P[o_{t+1},\dotsb,o_{\tau}|h_{t+1}=i]$ by multiplying $O^{(t)}$ by $m^{\tau-t}$ and dividing $E^{(t)}$ by $m^{\tau-t}$. Let the normalized matrices be $\tilde{O}^{(t)}$ and $\tilde{E}^{(t)}$. Therefore,
		\begin{align}
		&\tilde{O}^{(t)}_{i,i} \le \Big(1+\sqrt{\frac{24m\log^3 n}{d}}\Big)\nonumber\\
		m\Big(1-\sqrt{\frac{24m\log^3 n}{2d}}\Big)\le &\tilde{E}^{(t)}_{i,i}\le m\Big(1+\sqrt{\frac{12m\log^3 n}{d}}\Big)  \nonumber
		\end{align}
		
		Consider any $x$ such that $1^{T}x=0$ and $\norm{x}=1$. Let $\tilde{E}^{(t)}x = \alpha v + x_2$, where $1^Tx_2=0, \norm{x_2}\le 1$ and $v$ is the all ones vector normalized to have unit $\ell_2$-norm. We claim that $\alpha = v^Tx \le \sqrt{\frac{100m^3\log^3 n}{2d}}$. As $|\tilde{E}_{i,i}-\tilde{E}_{j,j}| \le \sqrt{\frac{100m^3\log^3 n}{2d}}$ for all $i\ne j$ and $1^Tx=0$, therefore
		\begin{align}
		|v^T\tilde{E}^{(t)}x| &\le \frac{\max_{i,j}|\tilde{E}_{i,i}-\tilde{E}_{j,j}|}{\sqrt{n}}\absnorm{x}\nonumber\\
		&\le \sqrt{\frac{100m^3\log^3 n}{2dn}}\absnorm{x}\le \sqrt{\frac{100m^3\log^3 n}{2d}}\norm{x}\le \sqrt{\frac{100m^3\log^3 n}{2d}}\nonumber
		\end{align}
		Therefore, $T\tilde{E}^{(t)}x=\alpha v+Tx_2$. Let the second eigenvalue of $T$ be upper bounded by $\lambda$. As $1^Tx_2=0$ therefore $\norm{Tx_2}\le \lambda$. Hence $\norm{T\tilde{E}^{(t)}x}\le \alpha + \lambda$ for any $x$ with $1^Tx=0$ and $\norm{x}=1$. Note that the operator norm of the matrix $\tilde{O}^{(t)}$ is at most $2$ because $\tilde{O}^{(t)}$ is a diagonal matrix with each entry bounded by $\Big(1+\sqrt{\frac{24m\log^3 n}{d}}\Big)\le 2$. Therefore $\norm{\tilde{O}T\tilde{E}^{(t)}x} \le 2(\alpha+\lambda)$ for any $x$ with $1^Tx=0$ and $\norm{x}=1$.
	\end{proof}
\end{proof}

==> NIPS Arxiv/main.tex <==
nips.tex

==> NIPS Arxiv/nips_learnability.tex <==
\vspace{-8pt}
\section{Learnability results for overcomplete HMMs}\label{sec:learnability}
\vspace{-8pt}
%The results in Section \ref{sec:identifiability} show that at least some HMMs with long term dependencies (such as when the transition matrix is a long cycle) are identifiable from short windows, but does not say anything about the sample complexities, and whether such HMMs can actually be learnt with number of samples being polynomial in the parameters. 

%For any distribution $p$, we define the $(1-\delta)$ support of $p$ to be the smallest set such that the total probability mass outside that set is at most $\delta$. 

%We now show that HMMs are learnable under some reasonable conditions on the transition matrix given generic observations. We first go over necessary definitions. Define $\sigma_{\min}^{(2)}(T)$ to be the minimum singular value of the transition matrix $T$. We also define
% We show that if the transition matrix has $\sigma_{\min}>0.1$, then the HMM is learnable upto error $\epsilon$ from $\poly{(k,d,\epsilon)}$ samples. Hence $\sigma_{\min}$ is a

%In order to learn from short windows (of length $O(\log_m n)$) we enforce an additional restriction on $T$ which intuitively means that the Markov Chain does not have small cycles and is hence not stuck in a small region of the state space for a long time. Under these restrictions,

In this section, we state our learnability result, discuss the assumptions and provide examples of HMMs which satisfy these assumptions. Our learnability results hold under the following conditions:
% Using tensor decomposition and the method of moments, we learn HMMs under the following conditions.  %\footnote{We also show slightly weaker learnability results under the $\ell_2$ norm.} --\\

\noindent \textbf{Assumptions:} For fixed constants $c_1, c_2, c_3 > 1 $, the HMM satisfies the following properties for some $c>0$:
\begin{enumerate}
%	\item \emph{Markov Chain is stationary:} $T$ has a stationary distribution, and every hidden state has stationary probability at least $1/\poly{n}$.
	\item \emph{Transition matrix is well-conditioned:} Both $T$ and the transition matrix $T'$ of the time reversed Markov Chain are well-conditioned in the $\ell_1$-norm: $\sigma_{\min}^{(1)}(T),\sigma_{\min}^{(1)}(T') \ge 1/m^{ c/c_1}$%\footnote{$\sigma_{\min}^{(1)}(T)$ is defined as $\min_{x\in \mathbb{R}^n}\frac{\absnorm{Tx}}{\absnorm{x}}$. We also obtain slightly weaker results for }
	%We outline the conditions in Theorem \ref{thm:learnability_l1} and Corollary \ref{thm:learnability}.
	\item \emph{Transition matrix does not have short cycles:} For both $T$ and $T'$, every state visits at least $10 \log_m n$ states in $15 \log_m n$ time except with probability $\delta_1 \le 1/n^c$.
	%$\sigma_{\min}(T),\sigma_{\min}(T')>1/m^{1/20}$.
	\item \emph{All hidden states have small ``degree'':} There exists $\delta_2$ such that for every hidden state $i$, the transition distributions $T_i$ and $T'_i$ have cumulative mass at most $\delta_2$ on all but $d$ states, with $d \le m^{1/c_2}$ and $\delta_2 \le 1/n^c$. Hence this is a soft ``degree'' requirement.
	%The ``degree'' $d$ is the size of the minimum set such that the transition distributions $T_i$ and $T'_i$ have cumulative mass at most $\delta_2$ on all but $d$ states, with $d \le m^{1/c_2}$ and $\delta_2 \le 1/n^c$.
	%	There exists $\delta_2$ such that for every hidden state $i$, the transition distributions $T_i$ and $T'_i$ have cumulative mass at most $\delta_2$ on all but $d$ states, with $d \le m^{1/c_2}$ and $\delta_2 \le 1/n^c$.
  \item \emph{Output distributions are random and have small support %\pl{small output support wasn't mentioned before}
  	:} There exists $\delta_3$ such that for every hidden state $i$ the output distribution $O_i$ has cumulative mass at most $\delta_3$ on all but $k$ outputs, with $k\le m^{1/c_3}$ and $\delta_3 \le 1/n^c$. Also, the output distribution $O_i$ is drawn uniformly on these $k$ outputs.
\end{enumerate}

The constants $c_1, c_2, c_3$ are can be made explicit, for example, $c_1 = 20, c_2 = 16$ and $c_3 = 10$ works. Under these conditions, we show that HMMs can be learned using polynomially many samples:

\begin{restatable}{thm}{learn}\label{thm:learnability}
	If an HMM satisfies the above conditions, then with high probability over the choice of $O$, the parameters of the HMM are learnable to within additive error $\epsilon$ with observations over windows of length $2\tau +1, \tau = 15\log_m n$, with the sample complexity $\poly{n,1/\epsilon}$.
\end{restatable}
\noindent \emph{Proof sketch.} We refer the reader to Section \ref{coupling} for the high level idea. Here, we provide a proof sketch for a much simpler case than that considered in Theorem \ref{thm:learnability} (also see Fig. \ref{fig:coupling}). Recall that our main goal is to show that the likelihood matrix $A$ is well-conditioned. Assume for simplicity that the output distribution of each hidden state is deterministic so the output distribution only has support on one of the $m$ character. The character on which the output distribution of each hidden state is supported is assigned independently and uniformly at random from the output alphabet. Also assume that $\delta_1, \delta_2, \delta_3$ in the conditions for Theorem \ref{thm:learnability} are zero. Our proof steps are roughly as follows--
\begin{enumerate}
	\item Consider two random walks $m_1$ and $m_2$ on $T$ starting at disjoint sets of hidden states at time 0.
	\item We first show that any two sample paths of a random walk on $T$ over $\tau = 15\log_m n$ time steps, both of which visit $10\log_m n$ different states in $\tau$ time steps but never meet in $\tau$ time steps, emit a different sequence of observations with high probability over the randomness in $O$.
	\item Using the fact that the degree of each hidden state is small, we perform a union bound over all possible sample paths to show that with high probability over the choice of $O$, any two sample paths which do not meet in $\tau$ time steps emit a different sequence of observations.
	\item Consider any 2 sample paths $s_1$ and $s_2$ corresponding to the random walks $m_1$ and $m_2$ which emit the same sequence of observations $w$ over $\tau$ time steps. By point 3 above, they must meet at some time $t$. If the probability of emitting $w$ under the random walks $m_1$ and $m_2$ are $p_1$ and $p_2$ respectively and $p_1>p_2$, then we show that $(p_1-p_2)$ of the probability mass in $m_1$ can be coupled with $m_2$ as these sample paths intersect sample paths from $m_2$. This is the core of the argument. Also refer to Fig. \ref{fig:coupling}.
	\item Hence if the probability of emitting a sequence of observations $w$ under the random walks $m_1$ and $m_2$ is very similar for every sequence $w$, then there is a very good coupling of the random walks, which implies that the total variational distance between the distribution of the random walks after $\tau$ time steps must be small. But this is a contradiction as $(\sigma_{\min}^{(1)}(T))^\tau$ is large. The contradiction stems from the fact that the $\ell_1$ distance between $m_1$ and $m_2$ at time 0 is one (as they start at disjoint starting states) and hence the distance at time $\tau$ is at least $ (\sigma_{\min}^{(1)}(T))^\tau $.
\end{enumerate}\hfill $\square$
\begin{figure}[h]
	\centering
	\includegraphics[height=1.5in]{coupling.png}
	\caption{Consider two random walks $m_1$ and $m_2$ for 4 time steps with disjoint starting states and with sample paths $s_1$ and $s_2$ which visits the states \emph{\{a,b,c,d\}} and \emph{\{e,b,c,f\}} at times $\{0,1,2,3\}$ respectively. We show that any two sample paths that have the same output distribution must be at the same hidden state at some time step. For example, here $s_1$ and $s_2$ are simultaneously at states \emph{b} and \emph{c}. This means that the probability mass in the two random walks can be coupled, hence the variational distance between the random walks $m_1$ and $m_2$ must be small at the end. But this cannot be the case as $T$ is well-conditioned. Hence most sample paths of $m_1$ and $m_2$ must have different output distributions, which means that random walks $m_1$ and $m_2$ which start at disjoint states must have different output distributions, which implies that $A$ is well-conditioned.}
	\label{fig:coupling}
\end{figure}
%\noindent \textbf{Theorem ~\ref{thm:learnability}.} \emph{	If an HMM satisfies the above conditions, then with high probability over the choice of $O$, the parameters of the HMM are learnable to within additive error $\epsilon$ with observations over windows of length $2\tau +1, \tau = 15\log_m n$, with the sample complexity being $\poly{n,1/\epsilon}$.}

Appendix \ref{sec:learning_proof} also states a corollary of Theorem \ref{thm:learnability} in terms of the minimum singular value $\sigma_{\min}(T)$ of the matrix $T$, instead of $\sigma_{\min}^{(1)}(T)$. We discuss the conditions for Theorem \ref{thm:learnability} next, and subsequently provide examples of HMMs which satisfy these conditions. %We obtain tighter results using $\sigma_{\min}^{(1)}(T)$, and these naturally imply slightly weaker results for $\sigma_{\min}^{(2)}(T)$

%\emph{Box containing proof sketch to be added.}

%To plug in some parameters, for $m=100$ and $\alpha = 0.75$, our assumptions hold true for $\sigma_{\min}>0.8, d \le 2, k\le 3$. 
\subsection{Discussion of the assumptions}\label{subsec:assumptions}

%We now discuss our assumptions for Theorem \ref{thm:identifiability} to motivate that at least some of them seem necessary. 

\begin{figure}
	\centering
	\begin{subfigure}{0.4 \textwidth}
		\includegraphics[height=1.5in]{cycle_cond}
		\caption{The conditioning becomes worse\\ when cycles are smaller or when more\\ probability mass $\epsilon$ is put on short cycles.}
		\label{fig:cycle_cond}
	\end{subfigure}
	\begin{subfigure}{0.4 \textwidth}
		\includegraphics[height=1.5 in]{degree_cond}
		\caption{The conditioning becomes worse as the degree increases, and when more probabiltiy mass $\epsilon$ is put on the dense part of $T$.}
		\label{fig:degree_cond}
	\end{subfigure}
	\caption{Experiments to study the effect of sparsity and short cycles on the learnability of HMMs. The condition number of the likelihood matrix $A$ determines the stability or sample complexity of the method of moments approach. The condition numbers are averaged over 10 trials.}
\end{figure}

%\begin{enumerate}
		%	\item \emph{Markov Chain is stationary:} The constraint that every hidden state has stationary probability at least $1/\poly{n}$ is necessary as otherwise we might not even visit all states in $\poly{n}$ samples.
	
		\,1.\, \emph{Transition matrix is well-conditioned:}
		Note that singular transition matrices might not even be identifiable. Moreover, \citet{mossel2005learning} showed that learning HMMs with singular transition matrices is as hard as learning parity with noise, which is widely conjectured to be computationally hard. Hence, it is necessary to exclude at least some classes of ill-conditioned transition matrices.% from learnability results for HMMs.
	
	\,2.\, \emph{Transition matrix does not have short cycles:} Due to Proposition \ref{lem:iden_lower_bnd}, we know that a HMM might not even be identifiable from short windows if it is composed of a union of short cycles, hence we expect a similar condition for learning the HMM with polynomial samples; though there is a gap between the upper and lower bounds in terms of the probability mass which is allowed on the short cycles. We performed some simulations to understand how the length of cycles in the transition matrix and the probability mass assigned to short cycles affects the condition number of the likelihood matrix $A$; recall that the condition number of $A$ determines the stability of the method of moments approach. We take the number of hidden states $n=128$, and let $P_{128}$ be a cycle on the $n$ hidden states (as in Fig. \ref{fig:example2}). Let $P_c$ be a union of short cycles of length $c$ on the $n$ states (refer to Fig. \ref{fig:nonex2} for an example). We take the transition matrix to be $T=\epsilon P_c+(1-\epsilon) P_{128}$ for different values of $c$ and $\epsilon$. Fig. \ref{fig:cycle_cond} shows that the condition number of $A$ becomes worse and hence learning requires more samples if the cycles are shorter in length, and if more probability mass is assigned to the short cycles, hinting that our conditions are perhaps not be too stringent.
	
	\,3.\, \emph{All hidden states have a small degree:} Condition 3 in Theorem \ref{thm:learnability} can be reinterpreted as saying that the transition probabilities out of any hidden state must have mass at most $1/n^{1+c}$ on any hidden state except a set of $d$ hidden states, for any $c>0$. While this soft constraint is weaker than a hard constraint on the degree, it natural to ask whether any sparsity is necessary to learn HMMs. As above, we carry out simulations to understand how the degree affects the condition number of the likelihood matrix $A$. We consider transition matrices on $n=128$ hidden states which are a combination of a dense part and a cycle. Define $P_{128}$ to be a cycle as before. Define $G_{d}$ as the adjacency matrix of a directed regular graph with degree $d$. We take the transition matrix $T=\epsilon G_d +(1-\epsilon d)P_{128}$. Hence the transition distribution of every hidden state has mass $\epsilon$ on a set of $d$ neighbors, and the residual probability mass is assigned to the permutation $P_{128}$. Fig. \ref{fig:degree_cond} shows that the condition number of $A$ becomes worse as the degree $d$ becomes larger, and as more probability mass $\epsilon$ is assigned to the dense part $G_d$ of the transition matrix $T$, providing some weak  evidence for the necessity of Condition 3. Also, recall that Theorem \ref{thm:lower_bound} shows that HMMs where the transition matrix is a random walk on an undirected regular graph with large degree (degree polynomial in $n$) cannot be learned using polynomially many samples if $m$ is a constant with respect to $n$. However, such graphs have all eigenvalues except the first one to be less than $O(1/\sqrt{n})$, hence it is not clear if the hardness of learning depends on the large degree itself or is only due to $T$ being ill-conditioned. More concretely, we pose the following open question:
	
		\textbf{Open question:} Consider an HMM with a transition matrix $T=(1-\epsilon)P+\epsilon U$, where $P$ is the cyclic permutation on $n$ hidden states (such as in Fig. \ref{fig:example2}) and $U$ is a random walk on a undirected, regular graph with large degree (polynomial in $n$) and $\epsilon>0$ is a constant. Can this HMM be learned using polynomial samples when $m$ is small (constant) with respect to $n$? This example approximately preserves $\sigma_{\min}(T)$ by the addition of the permutation, and hence the difficulty is only due to the transition matrix having large degree.
	 %, as indicated by Theorem \ref{thm:learnability}. % Fig. \ref{fig:degree_cond} plots the condition number of the matrix $A$ when the transition matrix 
	
	% While this soft constraint is significantly weaker than a hard constraint on the degree, it natural to ask whether any sparsity is necessary to learn HMMs. Theorem \ref{thm:lower_bound} shows that HMMs where the transition matrix is a random walk on an undirected regular graph with large degree (degree polynomial in $n$) cannot be learned using polynomially many samples if $m$ is a constant with respect to $n$. However, such graphs have all eigenvalues except the first one to be less than $O(1/\sqrt{d})$, hence it is not clear if the hardness of learning depends on the large degree itself or is only due to $T$ being ill-conditioned. More precisely, we pose the following concrete open question:
	
	 \,4.\,\emph{Output distributions are random and have small support:} As discussed in the introduction, if we do not assume that the observation matrices are random, then even simple HMMs with a cycle or permutation as the transition matrix might require long windows even to become identifiable, see Fig. \ref{fig:worsrt_O}. Hence some assumptions on the output distribution do seem necessary for learning the model from short time windows, though our assumptions are probably not tight. For instance, the assumption that the output distributions have a small support makes learning easier as it leads to the outputs being more discriminative of the hidden states, but it is not clear that this is a necessary assumption. Ideally, we would like to prove our learnability results under a \emph{smoothed} model for $O$, where an adversary is allowed to see the transition matrix $T$ and pick any worst-case $O$, but random noise is then added to the output distributions, which limits the power of the adversary. We believe our results should hold under such a smoothed setting, but set this aside for future work.

	
	% If we do not assume that the observation matrices are random, then even simple HMMs with a cycle or permutation as the transition matrix might require long windows even to become identifiable, see Fig. \ref{fig:worsrt_O}. Hence some assumptions do seem necessary for learning the model from short time windows. Ideally, we would like to prove our learnability results under a \emph{smoothed} model for $O$, where an adversary is allowed to see the transition matrix $T$ and pick any worst-case $O$, but random noise is then added to the output distributions, which limits the power of the adversary. We believe our results should hold under such a smoothed setting, but set this aside for future work.
	
	\begin{figure}[h]
		\centering
		\centering
		\includegraphics[height=1in]{worst_case_O}
		\caption{Consider two HMMs with transition matrices being cycles on $n=16$ states with binary outputs, and outputs conditioned on the hidden states are deterministic. The states labeled as 0 always emit a 0 and the states labeled as 1 always emit a 1. The two HMMs are not distinguishable from windows of length less than 8. Hence with worst case $O$ even simple HMMs like the cycle could require long windows to even become identifiable.}
		\label{fig:worsrt_O}
	\end{figure}
	
%	We believe the condition on the output distributions of the hidden states being concentrated is due to weakness of our proof technique rather than a fundamental property. Ideally, we would want to get learnability results under a smoothed model for $O$, where an adversary is allowed to see the transition matrix $T$ and pick any worst-case $O$, but random noise is then added to the output distributions, which limits the power of the adversary. We believe our results should hold under such a smoothed setting, but set this aside for future work.
	
% \end{enumerate}
%\vspace{-4 pt}
\subsection{Examples of transition matrices which satisfy our assumptions}\label{subsec:examples}

We revisit the examples from Fig. \ref{fig:example2} and Fig. \ref{fig:example1}, showing that they satisfy our assumptions. %for Theorem \ref{thm:learnability}.

%\begin{enumerate}
	\,1.\, \emph{Transition matrices where the Markov Chain is a permutation:} If the Markov chain is a permutation with all cycles longer than $10\log_m n $ then the transition matrix obeys all the conditions for Theorem \ref{thm:learnability}. This is because all the singular values of a permutation are 1, the degree is 1 and all hidden states visit $10\log_m n $ different states in $15\log_m n $ time steps.
	
	\,2.\, \emph{Transition matrices which are random walks on graphs with small degree and large girth:} For directed graphs, Condition 2 can be equivalently stated as that the graph representation of the transition matrix has a large girth (girth of a graph is defined as the length of its shortest cycle). %We show that this is also true for undirected graphs and the probability that a random walk on an undirected graph with girth larger than $20\log_m n$ visits less than $10\log_m n$ states in $15\log_m n$ time steps is small. 
	
	%\begin{restatable}{lem}{undirectgirth}\label{girth_undirected}
		
%	\end{restatable}
	
	\,3.\, \emph{Transition matrices of factorial HMMs:} Factorial HMMs \cite{ghahramani1997factorial} %(see Fig. \ref{fig:factorial}) 
	factor the latent state at any time into $D$ dimensions, each of which independently evolves according to a Markov process (see Fig. \ref{fig:factorial}). For $D=2$, this is equivalent to saying that the hidden states are indexed by two labels $(i,j)$ and if $T_1$ and $T_2$ represent the transition matrices for the two dimensions, then $\Prob[(i_1,j_1)\rightarrow(i_2,j_2)]= T_1(i_2,i_1)T_2(j_2,j_1)$. This naturally models settings where there are multiple latent concepts which evolve independently. The following properties are easy to show:
%	, or the product of the respective transitions in the original transition matrices Consider two transition matrices $T_1$ and $T_2$ on $n$ hidden states. Define $T=T_1 \otimes T_2$ as the Kronecker product of the matrices $T_1$ and $T_2$. This is equivalent to defining an HMM on $n^2$ hidden states where the hidden states are indexed by two labels $(i,j)$ and $P[(i_1,j_1)\rightarrow(i_2,j_2)]= T(i_2,i_2)T(j_2,j_1)$, or the product of the respective transitions in the original transition matrices. The following properties are easy to show--
%	\begin{lemma}
%		Let $T$ be the transition matrix of a factorial HMM composed of two Markov Chains with transition matrices $T_1$ and $T_2$. Then,
\vspace{-4pt}
		\begin{enumerate}
		\item If either of $T_1$ or $T_2$ visit $N$ different states in $15\log_m n $ time steps with probability $(1-\delta)$, then $T$ visits $N$ different states in $15\log_m n $ time steps with probability $(1-\delta)$.
		\item $\sigma_{\min}(T) = \sigma_{\min}(T_1)\sigma_{\min}(T_2)$
		\item If all hidden states in $T_1$ and $T_2$ have mass at most $\delta$ on all but $d_1$ states and $d_2$ states respectively, then $T$ has mass at most $2\delta$ on all but $d_1d_2$ states.
		%\item If $(1-\delta)$-support of $T_1 \le d_1$ and $(1-\delta)$-support of $T_2 \le d_2$ then $(1-2\delta)$-support of $T\le  d_1d_2$.
	\end{enumerate}
	\vspace{-4pt}
	Therefore, factorial HMMs are learnable with random $O$ if the underlying processes obey conditions similar to the assumptions for Theorem \ref{thm:learnability}. If both $T_1$ and $T_2$ are well-conditioned and at least one of them does not have short cycles, and either has small degree, then $T$ is learnable with random $O$.
	% If $T_1$ is simply a permutation with no short cycles, then $T$ is learnable with random $O$ if $T_2$ is learnable with random $O$. %Factorial HMMs have had %If $T_1$ cyclically shifts the hidden state by 1 at every time step, then this can be thought of as the index $i$ in $(i,j)$ being time, hence this corresponds to a time inhomegeneous Markov chain. Due to Theorem \ref{thm:learnability} this is learnable with generic observations if the transition matrix at every time step obeys the conditions for Theorem \ref{thm:learnability}.
%  \pl{why does $T_1$ have to be restricted to have short cycles?}

	\begin{figure}[h]
			\centering
			\includegraphics[height=1.5in]{factorial2}
			\caption{Graphical model for a factorial HMM for $D=2$. The Markov chains $M^{(1)}$ and $M^{(2)}$ evolve independently, and the output at any time step is only dependent on the current states of the two Markov chains at that time step. Our conditions for learning such transition matrices transfer cleanly to conditions on the transition matrices of the underlying Markov chains $M^{(1)}$ and $M^{(2)}$.}
			\label{fig:factorial}
	\end{figure}

%\end{enumerate}
%
%\begin{figure}[h]
%	\centering
%	{
%	\subfigure{
%		\centering
%		\includegraphics[height=1.8in]{white}
%		\caption{HMM with the transition matrix being a random walk on a graph with small degree and no short cycles. This can be thought of as a crude model for speech, with the words representing hidden states and the output being phonemes.}
%}
%	\subfigure{
%		\centering
%		\includegraphics[height=1.8in]{white}
%		\caption{HMM with a permutation as the transition matrix. The HMM has high long-term dependence, as the hidden state in the present completely determines the hidden state at any future time step. Such an HMM can be thought of as a a topic model which cycles through a large collection of topics.}
%	}
%}
%	\caption{Examples of transition matrices which fit in our framework, and have connections to relevant practical settings}
%	\label{fig:examples}
%\end{figure}


==> NIPS Arxiv/setup_colt.tex <==
\section{Discussion on tensor decomposition and method of moments for learning HMMs}\label{sec:tensor_basics}

We begin with some notation and basic facts about tensor decomposition in Section \ref{subsec:tensor}. We will follow by outlining the well-known tensor decomposition based approach to HMM learning in Section \ref{subsec:hmm_tensor}.

\subsection{Tensor preliminaries}\label{subsec:tensor}

Given a 3rd order rank $k$ tensor $M\in \Real^{d_1\times d_2 \times d_3}$, it can be written in terms of its factor matrices $A,B$ and $C$:
\begin{align}
M = \sum_{i\in [k]}^{} A_i \otimes B_i \otimes C_i  \nonumber
\end{align}
where $A_i$ denotes the $i$th column of a matrix $A$. Here $\otimes$ denotes the tensor product: if $a,b,c \in \mathbb{R}^d$ then $a \otimes b \otimes c \in \mathbb{R}^{d\times d \times d}$ and $(a \otimes b \otimes c)_{ijk}=a_i b_j c_k$. We refer to different dimensions of a tensor as the \emph{modes} of the tensor.

We denote $M_{(k)}$ as the mode $k$ matricization of the tensor, which is the flattening of the tensor along the $k$th direction obtained by stacking all the matrix slices together. For example $T_{(1)}$ denotes flattening of a tensor $T\in \mathbb{R}^{n \times m \times p}$ to a $(n \times mp)$ matrix. Recall that we denote the Khatri-Rao product of two matrices $A$ and $B$ as $(A \odot B )_i = (A_i \otimes B_i)_{(1)}$, where $(A_i \otimes B_i)_{(1)}$ denotes the flattening of the matrix $A_i \otimes B_i$ into a row vector. We denote the set $\{1,2,\dotsb,k\}=[k]$. 

Kruskal's condition \cite{kruskal1977three} says that if $A$ and $B$ are full rank and no two rows of $C$ are linearly dependent, then $M$ can be efficiently decomposed into the factors $A,B,C$ and the decomposition is unique upto scaling and permutation. The simultaneous decomposition algorithm \cite{chang1996full,leurgans1993decomposition} (Algorithm \ref{alg:learn_tensor}), is a well known algorithm to decompose tensors which satisfy Kruskal's condition.

%Therefore, if we can express the transition and observation matrices of the HMM as the factors of some tensor of empirical moments, then uniqueness of tensor decomposition will guarantee unique recovery of the transition and observation matrices. This is the well-known method-of-moments approach to parameter learning. 

%The simultaneous decomposition algorithm \cite{chang1996full,leurgans1993decomposition} (Algorithm \ref{alg:learn_tensor}), is a well known algorithm to decompose tensors which satisfy Kruskal's condition. Additionally, \citet{bhaskara2014smoothed} analyzed the sample complexity of the algorithm and showed that the number of samples needed is polynomial in $(k,1/\delta,\kappa)$, where $\delta$ is the separation between the closest eigenvalues of $M_a(M_b)^{-1}$ and $M_b(M_a)^{-1}$ and $\kappa$ is the maximum of the condition numbers of ${A}$ and ${B}$. We will use these perturbation bounds to get sample complexity bounds for learning.

\subsection{Learning HMMs using tensor decomposition}\label{subsec:hmm_tensor}

%An HMM is a model where the underlying or hidden state at each time step evolves according to Markov dynamics and the output at each time step only depends on the present hidden state. 
%We will reference the output at time $t$ by $y_t$ and hidden state at time $t$ as $h_t$. Let the number of hidden states be $n$ and the number of observations be $m$. As noted earlier, we are interested in the setting where $m \ll n$. 
The transition matrix $T\in \Real^{n\times n}$ for the HMM is defined as follows-
\begin{align}
\Prob[h_{t+1}=i|h_t = j] = T_{i,j} \;\forall \;i,j \nonumber
\end{align} 
The observation matrix $O\in \Real^{m\times n}$ is the probability of observing each output conditioned on the hidden state-
\begin{align}
\Prob[y_t = i | h_t = j] = O_{i,j} \;\forall \; i,j \nonumber
\end{align}
Also, given the transition matrix $T$, we define $T'$ as the time reversed Markov Chain. If the Markov Chain is time-reversible then $T=T'$.%, this is equivalent to saying that the Markov Chain is a random walk on a weighted, undirected graph.

%There has been a lot of work on learning HMMs and other latent variable models through tensor decomposition \cite{anandkumar13tensor}\cite{huang14hmm}. 
Our framework for HMM learning via tensor decomposition is identical to \citet{huang14hmm}. Algorithm \ref{alg:learn_tensor} describes how to compute $T$ and $O$ from the factors $A,B$ and $C$, we refer the reader to \citet{huang14hmm} for more details. 

%Note that $A$ is the likelihood of observing each sequence of observation conditioned on starting at a given hidden state. We'll refer to $A$ as the \emph{likelihood matrix} for this reason. $B$ is the equivalent matrix for the time-reversed Markov chain. If we show that $A,B$ and $C$ are full rank, then the HMM can be learned provided the exact moments, or infinite data. We do this in Section \ref{sec:identifiability}. Subsequently in Section \ref{sec:learnability}, we show that the matrices are well-conditioned, which implies learnability from polynomial samples. 

%We can similarly define $A^{(t-1)}$ as the likelihood matrix over $t-1$ steps--
%$$A_{L(l_1^{t-1}),i}^{(t-1)} = \Prob(y_1^{t-1}= l_1^{t-1} | x_0 = i)$$


%Note that $$C_{l,i} = \Prob(y_0 = l, x_0 = i)= \Prob(y_0=l|x_0=i)\Prob(x_0=i)$$ Hence  $O$ can be directly computed from $C$ as follows-
%\begin{align}
% O_{[:,i]} = C_{:,i}/(e^{T}C_{[:,i]})\nonumber
%\end{align}
%%$$A_{L(l_1^{t-1}),i}^{(t-1)} = \Prob(y_1^{t-1}= l_1^{t-1} | x_0 = i)$$
%Note that $$\Prob(y_1^t = l_1^t | x_0 = i) = \sum_{j}^{}\Prob(y_2^{t} = l_2^t | x_1 = j)\Prob(y_1 = l_1 | x_1 = j) \Prob(x_1 = j | x_0 = i) $$ which can be rewritten as $(O\odot A^{(n-1)})T = A$. This gives us a formula to estimate $T$ from $A, A_{n-1}$ and $O$
%\begin{align}	
% (O\odot A^{(t-1)})T = A \nonumber\\
% \implies &T = (O\odot A^{(t-1)})^\dagger A \label{T_est}
%\end{align}
%where $X^\dagger$ denotes the pseudo-inverse of $X$. Note that $A^{(n-1)}$ can be computed from $A$ by marginalizing the distribution over the last time step. The entire algorithm is summarized in Algorithm \ref{alg:learn_tensor}.

%Note that the time complexity of the algorithm is exponential in the window length $t$. Therefore, our goal is to determine the minimal window size over which we must estimate the joint probabilities of observations in order to be able to learn the model with polynomial sample complexity. This is also referred to as the HMM realization problem in the literature.

\begin{algorithm*}
	\caption{Learning HMMs with $m \ll n$ \cite{huang14hmm}}
	\label{alg:learn_tensor}
	\textbf{Input: }Moment tensor $M\in \Real^{m^\tau\times m^\tau \times m}$ over a window of length $\tau$\\
	\textbf{Output: }Estimates $\hat{T}$ and $\hat{O}$\\
	
	\textbf{Tensor decomposition using simultaneous diagonalization: }
	\begin{enumerate}
		
		\item Choose $a, b\in\Real^{d}$ uniformly at random. Project $M$ along the 3rd dimension to obtain $X, Y$ with $ X_{i,j} = \sum_{k}^{}M_{i,j,k}a_k$ and $Y_{i,j} = \sum_{k}^{}M_{i,j,k}b_k$. 
			\item Compute the eigendecomposition of $X(Y)^{-1}$ and $Y(X)^{-1}$. Let the columns of $A$ and $B$ to be the eigenvectors of $X(Y)^{-1}$ and $Y(X)^{-1}$ respectively. Pair them corresponding to reciprocal eigenvalues, and scale $A$ and $B$ to be column-stochastic.
\item Let ${M}_{(3)}\in \Real^{d^{2\tau}\times d}$ be the mode 3 matricization of $M$. Set ${C= {M}_{(3)}((A\odot B)^\dagger)^T}$.
\end{enumerate}

\textbf{Estimating $T$ and $O$ from tensor factors: }
\begin{enumerate}
\item Estimate $O$ by normalizing $C$ to be stochastic, i.e. $\hat{O}_{[:,i]} = C_{:,i}/(e^{T}C_{[:,i]})$ for all $i$.
\item Marginalize $A$ over the final time step to obtain $A^{(\tau-1)}$.
\item Estimate ${T}= (O\odot A^{(\tau-1)})^\dagger A$, 
	\end{enumerate}
\end{algorithm*}
%\begin{algorithm}
%	\caption{Learning HMMs with $m \\ n$}
%	\label{alg:learn_tensor}
%	\textbf{Input: }Moment tensor $M\in \Real^{d^n\times d^n \times d}$\\
%	\textbf{Output: }Factors $A\in \Real^{d^n\times k}, B \in \Real^{d^n\times k}, C \in \Real^{d\times k}$
%	\begin{enumerate}
%		\item Choose $a, b\in\Real^{d}$ uniformly at random. Project $M$ along the 3rd dimension to obtain $M_a = M(I,I,a)$ and $M_b = M(I,I,b)$. 
%		\item Compute the eigendecomposition of $M_a(M_b)^{-1}$ and $M_b(M_a)^{-1}$. Let the columns of $A$ and $B$ to be the eigenvectors of $M_a(M_b)^{-1}$ and $M_b(M_a)^{-1}$ respectively. Pair them corresponding to reciprocal eigenvalues, and scale $A$ and $B$ to be column-stochastic.
%		\item Let $\bar{M}_3\in \Real^{d^{2n}\times d}$ be the 3rd dimension matricization of $M$. Set $C= \bar{M}_3((A\odot)^\dagger)^T$.
%	\end{enumerate}
%\end{algorithm}

==> NIPS Arxiv/std-macros.tex <==
%%% THIS FILE IS AUTOMATICALLY GENERATED.  DON'T MODIFY, OR YOUR CHANGES MIGHT BE OVERWRITTEN!
\newcommand\sa{\ensuremath{\mathcal{a}}}
\newcommand\sd{\ensuremath{\mathcal{d}}}
\newcommand\se{\ensuremath{\mathcal{e}}}
\newcommand\sg{\ensuremath{\mathcal{g}}}
\newcommand\sh{\ensuremath{\mathcal{h}}}
\newcommand\si{\ensuremath{\mathcal{i}}}
\newcommand\sj{\ensuremath{\mathcal{j}}}
\newcommand\sk{\ensuremath{\mathcal{k}}}
\newcommand\sm{\ensuremath{\mathcal{m}}}
\newcommand\sn{\ensuremath{\mathcal{n}}}
\newcommand\so{\ensuremath{\mathcal{o}}}
\newcommand\sq{\ensuremath{\mathcal{q}}}
\newcommand\sr{\ensuremath{\mathcal{r}}}
\newcommand\st{\ensuremath{\mathcal{t}}}
\newcommand\su{\ensuremath{\mathcal{u}}}
\newcommand\sv{\ensuremath{\mathcal{v}}}
\newcommand\sw{\ensuremath{\mathcal{w}}}
\newcommand\sx{\ensuremath{\mathcal{x}}}
\newcommand\sy{\ensuremath{\mathcal{y}}}
\newcommand\sz{\ensuremath{\mathcal{z}}}
\newcommand\sA{\ensuremath{\mathcal{A}}}
\newcommand\sB{\ensuremath{\mathcal{B}}}
\newcommand\sC{\ensuremath{\mathcal{C}}}
\newcommand\sD{\ensuremath{\mathcal{D}}}
\newcommand\sE{\ensuremath{\mathcal{E}}}
\newcommand\sF{\ensuremath{\mathcal{F}}}
\newcommand\sG{\ensuremath{\mathcal{G}}}
\newcommand\sH{\ensuremath{\mathcal{H}}}
\newcommand\sI{\ensuremath{\mathcal{I}}}
\newcommand\sJ{\ensuremath{\mathcal{J}}}
\newcommand\sK{\ensuremath{\mathcal{K}}}
\newcommand\sL{\ensuremath{\mathcal{L}}}
\newcommand\sM{\ensuremath{\mathcal{M}}}
\newcommand\sN{\ensuremath{\mathcal{N}}}
\newcommand\sO{\ensuremath{\mathcal{O}}}
\newcommand\sP{\ensuremath{\mathcal{P}}}
\newcommand\sQ{\ensuremath{\mathcal{Q}}}
\newcommand\sR{\ensuremath{\mathcal{R}}}
\newcommand\sS{\ensuremath{\mathcal{S}}}
\newcommand\sT{\ensuremath{\mathcal{T}}}
\newcommand\sU{\ensuremath{\mathcal{U}}}
\newcommand\sV{\ensuremath{\mathcal{V}}}
\newcommand\sW{\ensuremath{\mathcal{W}}}
\newcommand\sX{\ensuremath{\mathcal{X}}}
\newcommand\sY{\ensuremath{\mathcal{Y}}}
\newcommand\sZ{\ensuremath{\mathcal{Z}}}
\newcommand\ba{\ensuremath{\mathbf{a}}}
\newcommand\bb{\ensuremath{\mathbf{b}}}
\newcommand\bc{\ensuremath{\mathbf{c}}}
\newcommand\bd{\ensuremath{\mathbf{d}}}
\newcommand\be{\ensuremath{\mathbf{e}}}
\newcommand\bg{\ensuremath{\mathbf{g}}}
\newcommand\bh{\ensuremath{\mathbf{h}}}
\newcommand\bi{\ensuremath{\mathbf{i}}}
\newcommand\bj{\ensuremath{\mathbf{j}}}
\newcommand\bk{\ensuremath{\mathbf{k}}}
\newcommand\bl{\ensuremath{\mathbf{l}}}
\newcommand\bn{\ensuremath{\mathbf{n}}}
\newcommand\bo{\ensuremath{\mathbf{o}}}
\newcommand\bp{\ensuremath{\mathbf{p}}}
\newcommand\bq{\ensuremath{\mathbf{q}}}
\newcommand\br{\ensuremath{\mathbf{r}}}
\newcommand\bs{\ensuremath{\mathbf{s}}}
\newcommand\bt{\ensuremath{\mathbf{t}}}
\newcommand\bu{\ensuremath{\mathbf{u}}}
\newcommand\bv{\ensuremath{\mathbf{v}}}
\newcommand\bw{\ensuremath{\mathbf{w}}}
\newcommand\bx{\ensuremath{\mathbf{x}}}
\newcommand\by{\ensuremath{\mathbf{y}}}
\newcommand\bz{\ensuremath{\mathbf{z}}}
\newcommand\bA{\ensuremath{\mathbf{A}}}
\newcommand\bB{\ensuremath{\mathbf{B}}}
\newcommand\bC{\ensuremath{\mathbf{C}}}
\newcommand\bD{\ensuremath{\mathbf{D}}}
\newcommand\bE{\ensuremath{\mathbf{E}}}
\newcommand\bF{\ensuremath{\mathbf{F}}}
\newcommand\bG{\ensuremath{\mathbf{G}}}
\newcommand\bH{\ensuremath{\mathbf{H}}}
\newcommand\bI{\ensuremath{\mathbf{I}}}
\newcommand\bJ{\ensuremath{\mathbf{J}}}
\newcommand\bK{\ensuremath{\mathbf{K}}}
\newcommand\bL{\ensuremath{\mathbf{L}}}
\newcommand\bM{\ensuremath{\mathbf{M}}}
\newcommand\bN{\ensuremath{\mathbf{N}}}
\newcommand\bO{\ensuremath{\mathbf{O}}}
\newcommand\bP{\ensuremath{\mathbf{P}}}
\newcommand\bQ{\ensuremath{\mathbf{Q}}}
\newcommand\bR{\ensuremath{\mathbf{R}}}
\newcommand\bS{\ensuremath{\mathbf{S}}}
\newcommand\bT{\ensuremath{\mathbf{T}}}
\newcommand\bU{\ensuremath{\mathbf{U}}}
\newcommand\bV{\ensuremath{\mathbf{V}}}
\newcommand\bW{\ensuremath{\mathbf{W}}}
\newcommand\bX{\ensuremath{\mathbf{X}}}
\newcommand\bY{\ensuremath{\mathbf{Y}}}
\newcommand\bZ{\ensuremath{\mathbf{Z}}}
\newcommand\Ba{\ensuremath{\mathbb{a}}}
\newcommand\Bb{\ensuremath{\mathbb{b}}}
\newcommand\Bc{\ensuremath{\mathbb{c}}}
\newcommand\Bd{\ensuremath{\mathbb{d}}}
\newcommand\Be{\ensuremath{\mathbb{e}}}
\newcommand\Bf{\ensuremath{\mathbb{f}}}
\newcommand\Bg{\ensuremath{\mathbb{g}}}
\newcommand\Bh{\ensuremath{\mathbb{h}}}
\newcommand\Bi{\ensuremath{\mathbb{i}}}
\newcommand\Bj{\ensuremath{\mathbb{j}}}
\newcommand\Bk{\ensuremath{\mathbb{k}}}
\newcommand\Bl{\ensuremath{\mathbb{l}}}
\newcommand\Bm{\ensuremath{\mathbb{m}}}
\newcommand\Bn{\ensuremath{\mathbb{n}}}
\newcommand\Bo{\ensuremath{\mathbb{o}}}
\newcommand\Bp{\ensuremath{\mathbb{p}}}
\newcommand\Bq{\ensuremath{\mathbb{q}}}
\newcommand\Br{\ensuremath{\mathbb{r}}}
\newcommand\Bs{\ensuremath{\mathbb{s}}}
\newcommand\Bt{\ensuremath{\mathbb{t}}}
\newcommand\Bu{\ensuremath{\mathbb{u}}}
\newcommand\Bv{\ensuremath{\mathbb{v}}}
\newcommand\Bw{\ensuremath{\mathbb{w}}}
\newcommand\Bx{\ensuremath{\mathbb{x}}}
\newcommand\By{\ensuremath{\mathbb{y}}}
\newcommand\Bz{\ensuremath{\mathbb{z}}}
\newcommand\BA{\ensuremath{\mathbb{A}}}
\newcommand\BB{\ensuremath{\mathbb{B}}}
\newcommand\BC{\ensuremath{\mathbb{C}}}
\newcommand\BD{\ensuremath{\mathbb{D}}}
\newcommand\BE{\ensuremath{\mathbb{E}}}
\newcommand\BF{\ensuremath{\mathbb{F}}}
\newcommand\BG{\ensuremath{\mathbb{G}}}
\newcommand\BH{\ensuremath{\mathbb{H}}}
\newcommand\BI{\ensuremath{\mathbb{I}}}
\newcommand\BJ{\ensuremath{\mathbb{J}}}
\newcommand\BK{\ensuremath{\mathbb{K}}}
\newcommand\BL{\ensuremath{\mathbb{L}}}
\newcommand\BM{\ensuremath{\mathbb{M}}}
\newcommand\BN{\ensuremath{\mathbb{N}}}
\newcommand\BO{\ensuremath{\mathbb{O}}}
\newcommand\BP{\ensuremath{\mathbb{P}}}
\newcommand\BQ{\ensuremath{\mathbb{Q}}}
\newcommand\BR{\ensuremath{\mathbb{R}}}
\newcommand\BS{\ensuremath{\mathbb{S}}}
\newcommand\BT{\ensuremath{\mathbb{T}}}
\newcommand\BU{\ensuremath{\mathbb{U}}}
\newcommand\BV{\ensuremath{\mathbb{V}}}
\newcommand\BW{\ensuremath{\mathbb{W}}}
\newcommand\BX{\ensuremath{\mathbb{X}}}
\newcommand\BY{\ensuremath{\mathbb{Y}}}
\newcommand\BZ{\ensuremath{\mathbb{Z}}}
\newcommand\balpha{\ensuremath{\mbox{\boldmath$\alpha$}}}
\newcommand\bbeta{\ensuremath{\mbox{\boldmath$\beta$}}}
\newcommand\btheta{\ensuremath{\mbox{\boldmath$\theta$}}}
\newcommand\bphi{\ensuremath{\mbox{\boldmath$\phi$}}}
\newcommand\bpi{\ensuremath{\mbox{\boldmath$\pi$}}}
\newcommand\bpsi{\ensuremath{\mbox{\boldmath$\psi$}}}
\newcommand\bmu{\ensuremath{\mbox{\boldmath$\mu$}}}
% Figures
\newcommand\fig[1]{\begin{center} \includegraphics{#1} \end{center}}
\newcommand\Fig[4]{\begin{figure}[ht] \begin{center} \includegraphics[scale=#2]{#1} \end{center} \caption{\label{fig:#3} #4} \end{figure}}
\newcommand\FigTop[4]{\begin{figure}[t] \begin{center} \includegraphics[scale=#2]{#1} \end{center} \caption{\label{fig:#3} #4} \end{figure}}
\newcommand\FigStar[4]{\begin{figure*}[ht] \begin{center} \includegraphics[scale=#2]{#1} \end{center} \caption{\label{fig:#3} #4} \end{figure*}}
\newcommand\FigRight[4]{\begin{wrapfigure}{r}{0.5\textwidth} \begin{center} \includegraphics[width=0.5\textwidth]{#1} \end{center} \caption{\label{fig:#3} #4} \end{wrapfigure}}
\newcommand\aside[1]{\quad\text{[#1]}}
\newcommand\interpret[1]{\llbracket #1 \rrbracket} % Denotation
% operators
\DeclareMathOperator*{\tr}{tr}
\DeclareMathOperator*{\sign}{sign}
\newcommand{\var}{\text{Var}} % Variance
\newcommand{\cov}{\text{Cov}} % Covariance
\DeclareMathOperator*{\diag}{diag} % Diagonal matrix
\newcommand\p[1]{\ensuremath{\left( #1 \right)}} % Parenthesis ()
\newcommand\pa[1]{\ensuremath{\left\langle #1 \right\rangle}} % <>
\newcommand\pb[1]{\ensuremath{\left[ #1 \right]}} % []
\newcommand\pc[1]{\ensuremath{\left\{ #1 \right\}}} % {}
\newcommand\eval[2]{\ensuremath{\left. #1 \right|_{#2}}} % Integral evaluation
\newcommand\inv[1]{\ensuremath{\frac{1}{#1}}}
\newcommand\half{\ensuremath{\frac{1}{2}}}
\newcommand\R{\ensuremath{\mathbb{R}}} % Real numbers
\newcommand\Z{\ensuremath{\mathbb{Z}}} % Integers
\newcommand\inner[2]{\ensuremath{\left< #1, #2 \right>}} % Inner product
\newcommand\mat[2]{\ensuremath{\left(\begin{array}{#1}#2\end{array}\right)}} % Matrix
\newcommand\eqn[1]{\begin{align} #1 \end{align}} % Equation (array)
\newcommand\eqnl[2]{\begin{align} \label{eqn:#1} #2 \end{align}} % Equation (array) with label
\newcommand\eqdef{\ensuremath{\stackrel{\rm def}{=}}} % Equal by definition
\newcommand{\1}{\mathbb{I}} % Indicator (don't use \mathbbm{1} because bbm is not TrueType)
\newcommand{\bone}{\mathbf{1}} % for vector one
\newcommand{\bzero}{\mathbf{0}} % for vector zero
\newcommand\refeqn[1]{(\ref{eqn:#1})}
\newcommand\refeqns[2]{(\ref{eqn:#1}) and (\ref{eqn:#2})}
\newcommand\refchp[1]{Chapter~\ref{chp:#1}}
\newcommand\refsec[1]{Section~\ref{sec:#1}}
\newcommand\refsecs[2]{Sections~\ref{sec:#1} and~\ref{sec:#2}}
\newcommand\reffig[1]{Figure~\ref{fig:#1}}
\newcommand\reffigs[2]{Figures~\ref{fig:#1} and~\ref{fig:#2}}
\newcommand\reffigss[3]{Figures~\ref{fig:#1},~\ref{fig:#2}, and~\ref{fig:#3}}
\newcommand\reffigsss[4]{Figures~\ref{fig:#1},~\ref{fig:#2},~\ref{fig:#3}, and~\ref{fig:#4}}
\newcommand\reftab[1]{Table~\ref{tab:#1}}
\newcommand\refapp[1]{Appendix~\ref{sec:#1}}
\newcommand\refthm[1]{Theorem~\ref{thm:#1}}
\newcommand\refthms[2]{Theorems~\ref{thm:#1} and~\ref{thm:#2}}
\newcommand\reflem[1]{Lemma~\ref{lem:#1}}
\newcommand\reflems[2]{Lemmas~\ref{lem:#1} and~\ref{lem:#2}}
\newcommand\refalg[1]{Algorithm~\ref{alg:#1}}
\newcommand\refalgs[2]{Algorithms~\ref{alg:#1} and~\ref{alg:#2}}
\newcommand\refex[1]{Example~\ref{ex:#1}}
\newcommand\refexs[2]{Examples~\ref{ex:#1} and~\ref{ex:#2}}
\newcommand\refprop[1]{Proposition~\ref{prop:#1}}
\newcommand\refdef[1]{Definition~\ref{def:#1}}
\newcommand\refcor[1]{Corollary~\ref{cor:#1}}
\newcommand\Chapter[2]{\chapter{#2}\label{chp:#1}}
\newcommand\Section[2]{\section{#2}\label{sec:#1}}
\newcommand\Subsection[2]{\subsection{#2}\label{sec:#1}}
\newcommand\Subsubsection[2]{\subsubsection{#2}\label{sec:#1}}
\ifthenelse{\isundefined{\definition}}{\newtheorem{definition}{Definition}}{}
\ifthenelse{\isundefined{\assumption}}{\newtheorem{assumption}{Assumption}}{}
\ifthenelse{\isundefined{\hypothesis}}{\newtheorem{hypothesis}{Hypothesis}}{}
\ifthenelse{\isundefined{\proposition}}{\newtheorem{proposition}{Proposition}}{}
\ifthenelse{\isundefined{\theorem}}{\newtheorem{theorem}{Theorem}}{}
\ifthenelse{\isundefined{\lemma}}{\newtheorem{lemma}{Lemma}}{}
\ifthenelse{\isundefined{\corollary}}{\newtheorem{corollary}{Corollary}}{}
\ifthenelse{\isundefined{\alg}}{\newtheorem{alg}{Algorithm}}{}
\ifthenelse{\isundefined{\example}}{\newtheorem{example}{Example}}{}
\newcommand\cv{\ensuremath{\to}} % Convergence
\newcommand\cvL{\ensuremath{\xrightarrow{\mathcal{L}}}} % Convergence in law
\newcommand\cvd{\ensuremath{\xrightarrow{d}}} % Convergence in distribution
\newcommand\cvP{\ensuremath{\xrightarrow{P}}} % Convergence in probability
\newcommand\cvas{\ensuremath{\xrightarrow{a.s.}}} % Convergence almost surely
\newcommand\eqdistrib{\ensuremath{\stackrel{d}{=}}} % Equal in distribution
\newcommand{\E}{\ensuremath{\mathbb{E}}} % Expectation
\newcommand\KL[2]{\ensuremath{\text{KL}\left( #1 \| #2 \right)}} % KL-divergence


==> main.tex <==
nips.tex

==> setup_colt.tex <==
\section{Discussion on tensor decomposition and method of moments for learning HMMs}\label{sec:tensor_basics}

We begin with some notation and basic facts about tensor decomposition in Section \ref{subsec:tensor}. We will follow by outlining the well-known tensor decomposition based approach to HMM learning in Section \ref{subsec:hmm_tensor}.

\subsection{Tensor preliminaries}\label{subsec:tensor}

Given a 3rd order rank $k$ tensor $M\in \Real^{d_1\times d_2 \times d_3}$, it can be written in terms of its factor matrices $A,B$ and $C$:
\begin{align}
M = \sum_{i\in [k]}^{} A_i \otimes B_i \otimes C_i  \nonumber
\end{align}
where $A_i$ denotes the $i$th column of a matrix $A$. Here $\otimes$ denotes the tensor product: if $a,b,c \in \mathbb{R}^d$ then $a \otimes b \otimes c \in \mathbb{R}^{d\times d \times d}$ and $(a \otimes b \otimes c)_{ijk}=a_i b_j c_k$. We refer to different dimensions of a tensor as the \emph{modes} of the tensor.

We denote $M_{(k)}$ as the mode $k$ matricization of the tensor, which is the flattening of the tensor along the $k$th direction obtained by stacking all the matrix slices together. For example $T_{(1)}$ denotes flattening of a tensor $T\in \mathbb{R}^{n \times m \times p}$ to a $(n \times mp)$ matrix. Recall that we denote the Khatri-Rao product of two matrices $A$ and $B$ as $(A \odot B )_i = (A_i \otimes B_i)_{(1)}$, where $(A_i \otimes B_i)_{(1)}$ denotes the flattening of the matrix $A_i \otimes B_i$ into a row vector. We denote the set $\{1,2,\dotsb,k\}=[k]$. 

Kruskal's condition \cite{kruskal1977three} says that if $A$ and $B$ are full rank and no two rows of $C$ are linearly dependent, then $M$ can be efficiently decomposed into the factors $A,B,C$ and the decomposition is unique upto scaling and permutation. The simultaneous decomposition algorithm \cite{chang1996full,leurgans1993decomposition} (Algorithm \ref{alg:learn_tensor}), is a well known algorithm to decompose tensors which satisfy Kruskal's condition.

%Therefore, if we can express the transition and observation matrices of the HMM as the factors of some tensor of empirical moments, then uniqueness of tensor decomposition will guarantee unique recovery of the transition and observation matrices. This is the well-known method-of-moments approach to parameter learning. 

%The simultaneous decomposition algorithm \cite{chang1996full,leurgans1993decomposition} (Algorithm \ref{alg:learn_tensor}), is a well known algorithm to decompose tensors which satisfy Kruskal's condition. Additionally, \citet{bhaskara2014smoothed} analyzed the sample complexity of the algorithm and showed that the number of samples needed is polynomial in $(k,1/\delta,\kappa)$, where $\delta$ is the separation between the closest eigenvalues of $M_a(M_b)^{-1}$ and $M_b(M_a)^{-1}$ and $\kappa$ is the maximum of the condition numbers of ${A}$ and ${B}$. We will use these perturbation bounds to get sample complexity bounds for learning.

\subsection{Learning HMMs using tensor decomposition}\label{subsec:hmm_tensor}

%An HMM is a model where the underlying or hidden state at each time step evolves according to Markov dynamics and the output at each time step only depends on the present hidden state. 
%We will reference the output at time $t$ by $y_t$ and hidden state at time $t$ as $h_t$. Let the number of hidden states be $n$ and the number of observations be $m$. As noted earlier, we are interested in the setting where $m \ll n$. 
The transition matrix $T\in \Real^{n\times n}$ for the HMM is defined as follows-
\begin{align}
\Prob[h_{t+1}=i|h_t = j] = T_{i,j} \;\forall \;i,j \nonumber
\end{align} 
The observation matrix $O\in \Real^{m\times n}$ is the probability of observing each output conditioned on the hidden state-
\begin{align}
\Prob[y_t = i | h_t = j] = O_{i,j} \;\forall \; i,j \nonumber
\end{align}
Also, given the transition matrix $T$, we define $T'$ as the time reversed Markov Chain. If the Markov Chain is time-reversible then $T=T'$.%, this is equivalent to saying that the Markov Chain is a random walk on a weighted, undirected graph.

%There has been a lot of work on learning HMMs and other latent variable models through tensor decomposition \cite{anandkumar13tensor}\cite{huang14hmm}. 
Our framework for HMM learning via tensor decomposition is identical to \citet{huang14hmm}. Algorithm \ref{alg:learn_tensor} describes how to compute $T$ and $O$ from the factors $A,B$ and $C$, we refer the reader to \citet{huang14hmm} for more details. 

%Note that $A$ is the likelihood of observing each sequence of observation conditioned on starting at a given hidden state. We'll refer to $A$ as the \emph{likelihood matrix} for this reason. $B$ is the equivalent matrix for the time-reversed Markov chain. If we show that $A,B$ and $C$ are full rank, then the HMM can be learned provided the exact moments, or infinite data. We do this in Section \ref{sec:identifiability}. Subsequently in Section \ref{sec:learnability}, we show that the matrices are well-conditioned, which implies learnability from polynomial samples. 

%We can similarly define $A^{(t-1)}$ as the likelihood matrix over $t-1$ steps--
%$$A_{L(l_1^{t-1}),i}^{(t-1)} = \Prob(y_1^{t-1}= l_1^{t-1} | x_0 = i)$$


%Note that $$C_{l,i} = \Prob(y_0 = l, x_0 = i)= \Prob(y_0=l|x_0=i)\Prob(x_0=i)$$ Hence  $O$ can be directly computed from $C$ as follows-
%\begin{align}
% O_{[:,i]} = C_{:,i}/(e^{T}C_{[:,i]})\nonumber
%\end{align}
%%$$A_{L(l_1^{t-1}),i}^{(t-1)} = \Prob(y_1^{t-1}= l_1^{t-1} | x_0 = i)$$
%Note that $$\Prob(y_1^t = l_1^t | x_0 = i) = \sum_{j}^{}\Prob(y_2^{t} = l_2^t | x_1 = j)\Prob(y_1 = l_1 | x_1 = j) \Prob(x_1 = j | x_0 = i) $$ which can be rewritten as $(O\odot A^{(n-1)})T = A$. This gives us a formula to estimate $T$ from $A, A_{n-1}$ and $O$
%\begin{align}	
% (O\odot A^{(t-1)})T = A \nonumber\\
% \implies &T = (O\odot A^{(t-1)})^\dagger A \label{T_est}
%\end{align}
%where $X^\dagger$ denotes the pseudo-inverse of $X$. Note that $A^{(n-1)}$ can be computed from $A$ by marginalizing the distribution over the last time step. The entire algorithm is summarized in Algorithm \ref{alg:learn_tensor}.

%Note that the time complexity of the algorithm is exponential in the window length $t$. Therefore, our goal is to determine the minimal window size over which we must estimate the joint probabilities of observations in order to be able to learn the model with polynomial sample complexity. This is also referred to as the HMM realization problem in the literature.

\begin{algorithm*}
	\caption{Learning HMMs with $m \ll n$ \cite{huang14hmm}}
	\label{alg:learn_tensor}
	\textbf{Input: }Moment tensor $M\in \Real^{m^\tau\times m^\tau \times m}$ over a window of length $\tau$\\
	\textbf{Output: }Estimates $\hat{T}$ and $\hat{O}$\\
	
	\textbf{Tensor decomposition using simultaneous diagonalization: }
	\begin{enumerate}
		
		\item Choose $a, b\in\Real^{d}$ uniformly at random. Project $M$ along the 3rd dimension to obtain $X, Y$ with $ X_{i,j} = \sum_{k}^{}M_{i,j,k}a_k$ and $Y_{i,j} = \sum_{k}^{}M_{i,j,k}b_k$. 
			\item Compute the eigendecomposition of $X(Y)^{-1}$ and $Y(X)^{-1}$. Let the columns of $A$ and $B$ to be the eigenvectors of $X(Y)^{-1}$ and $Y(X)^{-1}$ respectively. Pair them corresponding to reciprocal eigenvalues, and scale $A$ and $B$ to be column-stochastic.
\item Let ${M}_{(3)}\in \Real^{d^{2\tau}\times d}$ be the mode 3 matricization of $M$. Set ${C= {M}_{(3)}((A\odot B)^\dagger)^T}$.
\end{enumerate}

\textbf{Estimating $T$ and $O$ from tensor factors: }
\begin{enumerate}
\item Estimate $O$ by normalizing $C$ to be stochastic, i.e. $\hat{O}_{[:,i]} = C_{:,i}/(e^{T}C_{[:,i]})$ for all $i$.
\item Marginalize $A$ over the final time step to obtain $A^{(\tau-1)}$.
\item Estimate ${T}= (O\odot A^{(\tau-1)})^\dagger A$, 
	\end{enumerate}
\end{algorithm*}
%\begin{algorithm}
%	\caption{Learning HMMs with $m \\ n$}
%	\label{alg:learn_tensor}
%	\textbf{Input: }Moment tensor $M\in \Real^{d^n\times d^n \times d}$\\
%	\textbf{Output: }Factors $A\in \Real^{d^n\times k}, B \in \Real^{d^n\times k}, C \in \Real^{d\times k}$
%	\begin{enumerate}
%		\item Choose $a, b\in\Real^{d}$ uniformly at random. Project $M$ along the 3rd dimension to obtain $M_a = M(I,I,a)$ and $M_b = M(I,I,b)$. 
%		\item Compute the eigendecomposition of $M_a(M_b)^{-1}$ and $M_b(M_a)^{-1}$. Let the columns of $A$ and $B$ to be the eigenvectors of $M_a(M_b)^{-1}$ and $M_b(M_a)^{-1}$ respectively. Pair them corresponding to reciprocal eigenvalues, and scale $A$ and $B$ to be column-stochastic.
%		\item Let $\bar{M}_3\in \Real^{d^{2n}\times d}$ be the 3rd dimension matricization of $M$. Set $C= \bar{M}_3((A\odot)^\dagger)^T$.
%	\end{enumerate}
%\end{algorithm}

==> std-macros.tex <==
%%% THIS FILE IS AUTOMATICALLY GENERATED.  DON'T MODIFY, OR YOUR CHANGES MIGHT BE OVERWRITTEN!
\newcommand\sa{\ensuremath{\mathcal{a}}}
\newcommand\sd{\ensuremath{\mathcal{d}}}
\newcommand\se{\ensuremath{\mathcal{e}}}
\newcommand\sg{\ensuremath{\mathcal{g}}}
\newcommand\sh{\ensuremath{\mathcal{h}}}
\newcommand\si{\ensuremath{\mathcal{i}}}
\newcommand\sj{\ensuremath{\mathcal{j}}}
\newcommand\sk{\ensuremath{\mathcal{k}}}
\newcommand\sm{\ensuremath{\mathcal{m}}}
\newcommand\sn{\ensuremath{\mathcal{n}}}
\newcommand\so{\ensuremath{\mathcal{o}}}
\newcommand\sq{\ensuremath{\mathcal{q}}}
\newcommand\sr{\ensuremath{\mathcal{r}}}
\newcommand\st{\ensuremath{\mathcal{t}}}
\newcommand\su{\ensuremath{\mathcal{u}}}
\newcommand\sv{\ensuremath{\mathcal{v}}}
\newcommand\sw{\ensuremath{\mathcal{w}}}
\newcommand\sx{\ensuremath{\mathcal{x}}}
\newcommand\sy{\ensuremath{\mathcal{y}}}
\newcommand\sz{\ensuremath{\mathcal{z}}}
\newcommand\sA{\ensuremath{\mathcal{A}}}
\newcommand\sB{\ensuremath{\mathcal{B}}}
\newcommand\sC{\ensuremath{\mathcal{C}}}
\newcommand\sD{\ensuremath{\mathcal{D}}}
\newcommand\sE{\ensuremath{\mathcal{E}}}
\newcommand\sF{\ensuremath{\mathcal{F}}}
\newcommand\sG{\ensuremath{\mathcal{G}}}
\newcommand\sH{\ensuremath{\mathcal{H}}}
\newcommand\sI{\ensuremath{\mathcal{I}}}
\newcommand\sJ{\ensuremath{\mathcal{J}}}
\newcommand\sK{\ensuremath{\mathcal{K}}}
\newcommand\sL{\ensuremath{\mathcal{L}}}
\newcommand\sM{\ensuremath{\mathcal{M}}}
\newcommand\sN{\ensuremath{\mathcal{N}}}
\newcommand\sO{\ensuremath{\mathcal{O}}}
\newcommand\sP{\ensuremath{\mathcal{P}}}
\newcommand\sQ{\ensuremath{\mathcal{Q}}}
\newcommand\sR{\ensuremath{\mathcal{R}}}
\newcommand\sS{\ensuremath{\mathcal{S}}}
\newcommand\sT{\ensuremath{\mathcal{T}}}
\newcommand\sU{\ensuremath{\mathcal{U}}}
\newcommand\sV{\ensuremath{\mathcal{V}}}
\newcommand\sW{\ensuremath{\mathcal{W}}}
\newcommand\sX{\ensuremath{\mathcal{X}}}
\newcommand\sY{\ensuremath{\mathcal{Y}}}
\newcommand\sZ{\ensuremath{\mathcal{Z}}}
\newcommand\ba{\ensuremath{\mathbf{a}}}
\newcommand\bb{\ensuremath{\mathbf{b}}}
\newcommand\bc{\ensuremath{\mathbf{c}}}
\newcommand\bd{\ensuremath{\mathbf{d}}}
\newcommand\be{\ensuremath{\mathbf{e}}}
\newcommand\bg{\ensuremath{\mathbf{g}}}
\newcommand\bh{\ensuremath{\mathbf{h}}}
\newcommand\bi{\ensuremath{\mathbf{i}}}
\newcommand\bj{\ensuremath{\mathbf{j}}}
\newcommand\bk{\ensuremath{\mathbf{k}}}
\newcommand\bl{\ensuremath{\mathbf{l}}}
\newcommand\bn{\ensuremath{\mathbf{n}}}
\newcommand\bo{\ensuremath{\mathbf{o}}}
\newcommand\bp{\ensuremath{\mathbf{p}}}
\newcommand\bq{\ensuremath{\mathbf{q}}}
\newcommand\br{\ensuremath{\mathbf{r}}}
\newcommand\bs{\ensuremath{\mathbf{s}}}
\newcommand\bt{\ensuremath{\mathbf{t}}}
\newcommand\bu{\ensuremath{\mathbf{u}}}
\newcommand\bv{\ensuremath{\mathbf{v}}}
\newcommand\bw{\ensuremath{\mathbf{w}}}
\newcommand\bx{\ensuremath{\mathbf{x}}}
\newcommand\by{\ensuremath{\mathbf{y}}}
\newcommand\bz{\ensuremath{\mathbf{z}}}
\newcommand\bA{\ensuremath{\mathbf{A}}}
\newcommand\bB{\ensuremath{\mathbf{B}}}
\newcommand\bC{\ensuremath{\mathbf{C}}}
\newcommand\bD{\ensuremath{\mathbf{D}}}
\newcommand\bE{\ensuremath{\mathbf{E}}}
\newcommand\bF{\ensuremath{\mathbf{F}}}
\newcommand\bG{\ensuremath{\mathbf{G}}}
\newcommand\bH{\ensuremath{\mathbf{H}}}
\newcommand\bI{\ensuremath{\mathbf{I}}}
\newcommand\bJ{\ensuremath{\mathbf{J}}}
\newcommand\bK{\ensuremath{\mathbf{K}}}
\newcommand\bL{\ensuremath{\mathbf{L}}}
\newcommand\bM{\ensuremath{\mathbf{M}}}
\newcommand\bN{\ensuremath{\mathbf{N}}}
\newcommand\bO{\ensuremath{\mathbf{O}}}
\newcommand\bP{\ensuremath{\mathbf{P}}}
\newcommand\bQ{\ensuremath{\mathbf{Q}}}
\newcommand\bR{\ensuremath{\mathbf{R}}}
\newcommand\bS{\ensuremath{\mathbf{S}}}
\newcommand\bT{\ensuremath{\mathbf{T}}}
\newcommand\bU{\ensuremath{\mathbf{U}}}
\newcommand\bV{\ensuremath{\mathbf{V}}}
\newcommand\bW{\ensuremath{\mathbf{W}}}
\newcommand\bX{\ensuremath{\mathbf{X}}}
\newcommand\bY{\ensuremath{\mathbf{Y}}}
\newcommand\bZ{\ensuremath{\mathbf{Z}}}
\newcommand\Ba{\ensuremath{\mathbb{a}}}
\newcommand\Bb{\ensuremath{\mathbb{b}}}
\newcommand\Bc{\ensuremath{\mathbb{c}}}
\newcommand\Bd{\ensuremath{\mathbb{d}}}
\newcommand\Be{\ensuremath{\mathbb{e}}}
\newcommand\Bf{\ensuremath{\mathbb{f}}}
\newcommand\Bg{\ensuremath{\mathbb{g}}}
\newcommand\Bh{\ensuremath{\mathbb{h}}}
\newcommand\Bi{\ensuremath{\mathbb{i}}}
\newcommand\Bj{\ensuremath{\mathbb{j}}}
\newcommand\Bk{\ensuremath{\mathbb{k}}}
\newcommand\Bl{\ensuremath{\mathbb{l}}}
\newcommand\Bm{\ensuremath{\mathbb{m}}}
\newcommand\Bn{\ensuremath{\mathbb{n}}}
\newcommand\Bo{\ensuremath{\mathbb{o}}}
\newcommand\Bp{\ensuremath{\mathbb{p}}}
\newcommand\Bq{\ensuremath{\mathbb{q}}}
\newcommand\Br{\ensuremath{\mathbb{r}}}
\newcommand\Bs{\ensuremath{\mathbb{s}}}
\newcommand\Bt{\ensuremath{\mathbb{t}}}
\newcommand\Bu{\ensuremath{\mathbb{u}}}
\newcommand\Bv{\ensuremath{\mathbb{v}}}
\newcommand\Bw{\ensuremath{\mathbb{w}}}
\newcommand\Bx{\ensuremath{\mathbb{x}}}
\newcommand\By{\ensuremath{\mathbb{y}}}
\newcommand\Bz{\ensuremath{\mathbb{z}}}
\newcommand\BA{\ensuremath{\mathbb{A}}}
\newcommand\BB{\ensuremath{\mathbb{B}}}
\newcommand\BC{\ensuremath{\mathbb{C}}}
\newcommand\BD{\ensuremath{\mathbb{D}}}
\newcommand\BE{\ensuremath{\mathbb{E}}}
\newcommand\BF{\ensuremath{\mathbb{F}}}
\newcommand\BG{\ensuremath{\mathbb{G}}}
\newcommand\BH{\ensuremath{\mathbb{H}}}
\newcommand\BI{\ensuremath{\mathbb{I}}}
\newcommand\BJ{\ensuremath{\mathbb{J}}}
\newcommand\BK{\ensuremath{\mathbb{K}}}
\newcommand\BL{\ensuremath{\mathbb{L}}}
\newcommand\BM{\ensuremath{\mathbb{M}}}
\newcommand\BN{\ensuremath{\mathbb{N}}}
\newcommand\BO{\ensuremath{\mathbb{O}}}
\newcommand\BP{\ensuremath{\mathbb{P}}}
\newcommand\BQ{\ensuremath{\mathbb{Q}}}
\newcommand\BR{\ensuremath{\mathbb{R}}}
\newcommand\BS{\ensuremath{\mathbb{S}}}
\newcommand\BT{\ensuremath{\mathbb{T}}}
\newcommand\BU{\ensuremath{\mathbb{U}}}
\newcommand\BV{\ensuremath{\mathbb{V}}}
\newcommand\BW{\ensuremath{\mathbb{W}}}
\newcommand\BX{\ensuremath{\mathbb{X}}}
\newcommand\BY{\ensuremath{\mathbb{Y}}}
\newcommand\BZ{\ensuremath{\mathbb{Z}}}
\newcommand\balpha{\ensuremath{\mbox{\boldmath$\alpha$}}}
\newcommand\bbeta{\ensuremath{\mbox{\boldmath$\beta$}}}
\newcommand\btheta{\ensuremath{\mbox{\boldmath$\theta$}}}
\newcommand\bphi{\ensuremath{\mbox{\boldmath$\phi$}}}
\newcommand\bpi{\ensuremath{\mbox{\boldmath$\pi$}}}
\newcommand\bpsi{\ensuremath{\mbox{\boldmath$\psi$}}}
\newcommand\bmu{\ensuremath{\mbox{\boldmath$\mu$}}}
% Figures
\newcommand\fig[1]{\begin{center} \includegraphics{#1} \end{center}}
\newcommand\Fig[4]{\begin{figure}[ht] \begin{center} \includegraphics[scale=#2]{#1} \end{center} \caption{\label{fig:#3} #4} \end{figure}}
\newcommand\FigTop[4]{\begin{figure}[t] \begin{center} \includegraphics[scale=#2]{#1} \end{center} \caption{\label{fig:#3} #4} \end{figure}}
\newcommand\FigStar[4]{\begin{figure*}[ht] \begin{center} \includegraphics[scale=#2]{#1} \end{center} \caption{\label{fig:#3} #4} \end{figure*}}
\newcommand\FigRight[4]{\begin{wrapfigure}{r}{0.5\textwidth} \begin{center} \includegraphics[width=0.5\textwidth]{#1} \end{center} \caption{\label{fig:#3} #4} \end{wrapfigure}}
\newcommand\aside[1]{\quad\text{[#1]}}
\newcommand\interpret[1]{\llbracket #1 \rrbracket} % Denotation
% operators
\DeclareMathOperator*{\tr}{tr}
\DeclareMathOperator*{\sign}{sign}
\newcommand{\var}{\text{Var}} % Variance
\newcommand{\cov}{\text{Cov}} % Covariance
\DeclareMathOperator*{\diag}{diag} % Diagonal matrix
\newcommand\p[1]{\ensuremath{\left( #1 \right)}} % Parenthesis ()
\newcommand\pa[1]{\ensuremath{\left\langle #1 \right\rangle}} % <>
\newcommand\pb[1]{\ensuremath{\left[ #1 \right]}} % []
\newcommand\pc[1]{\ensuremath{\left\{ #1 \right\}}} % {}
\newcommand\eval[2]{\ensuremath{\left. #1 \right|_{#2}}} % Integral evaluation
\newcommand\inv[1]{\ensuremath{\frac{1}{#1}}}
\newcommand\half{\ensuremath{\frac{1}{2}}}
\newcommand\R{\ensuremath{\mathbb{R}}} % Real numbers
\newcommand\Z{\ensuremath{\mathbb{Z}}} % Integers
\newcommand\inner[2]{\ensuremath{\left< #1, #2 \right>}} % Inner product
\newcommand\mat[2]{\ensuremath{\left(\begin{array}{#1}#2\end{array}\right)}} % Matrix
\newcommand\eqn[1]{\begin{align} #1 \end{align}} % Equation (array)
\newcommand\eqnl[2]{\begin{align} \label{eqn:#1} #2 \end{align}} % Equation (array) with label
\newcommand\eqdef{\ensuremath{\stackrel{\rm def}{=}}} % Equal by definition
\newcommand{\1}{\mathbb{I}} % Indicator (don't use \mathbbm{1} because bbm is not TrueType)
\newcommand{\bone}{\mathbf{1}} % for vector one
\newcommand{\bzero}{\mathbf{0}} % for vector zero
\newcommand\refeqn[1]{(\ref{eqn:#1})}
\newcommand\refeqns[2]{(\ref{eqn:#1}) and (\ref{eqn:#2})}
\newcommand\refchp[1]{Chapter~\ref{chp:#1}}
\newcommand\refsec[1]{Section~\ref{sec:#1}}
\newcommand\refsecs[2]{Sections~\ref{sec:#1} and~\ref{sec:#2}}
\newcommand\reffig[1]{Figure~\ref{fig:#1}}
\newcommand\reffigs[2]{Figures~\ref{fig:#1} and~\ref{fig:#2}}
\newcommand\reffigss[3]{Figures~\ref{fig:#1},~\ref{fig:#2}, and~\ref{fig:#3}}
\newcommand\reffigsss[4]{Figures~\ref{fig:#1},~\ref{fig:#2},~\ref{fig:#3}, and~\ref{fig:#4}}
\newcommand\reftab[1]{Table~\ref{tab:#1}}
\newcommand\refapp[1]{Appendix~\ref{sec:#1}}
\newcommand\refthm[1]{Theorem~\ref{thm:#1}}
\newcommand\refthms[2]{Theorems~\ref{thm:#1} and~\ref{thm:#2}}
\newcommand\reflem[1]{Lemma~\ref{lem:#1}}
\newcommand\reflems[2]{Lemmas~\ref{lem:#1} and~\ref{lem:#2}}
\newcommand\refalg[1]{Algorithm~\ref{alg:#1}}
\newcommand\refalgs[2]{Algorithms~\ref{alg:#1} and~\ref{alg:#2}}
\newcommand\refex[1]{Example~\ref{ex:#1}}
\newcommand\refexs[2]{Examples~\ref{ex:#1} and~\ref{ex:#2}}
\newcommand\refprop[1]{Proposition~\ref{prop:#1}}
\newcommand\refdef[1]{Definition~\ref{def:#1}}
\newcommand\refcor[1]{Corollary~\ref{cor:#1}}
\newcommand\Chapter[2]{\chapter{#2}\label{chp:#1}}
\newcommand\Section[2]{\section{#2}\label{sec:#1}}
\newcommand\Subsection[2]{\subsection{#2}\label{sec:#1}}
\newcommand\Subsubsection[2]{\subsubsection{#2}\label{sec:#1}}
\ifthenelse{\isundefined{\definition}}{\newtheorem{definition}{Definition}}{}
\ifthenelse{\isundefined{\assumption}}{\newtheorem{assumption}{Assumption}}{}
\ifthenelse{\isundefined{\hypothesis}}{\newtheorem{hypothesis}{Hypothesis}}{}
\ifthenelse{\isundefined{\proposition}}{\newtheorem{proposition}{Proposition}}{}
\ifthenelse{\isundefined{\theorem}}{\newtheorem{theorem}{Theorem}}{}
\ifthenelse{\isundefined{\lemma}}{\newtheorem{lemma}{Lemma}}{}
\ifthenelse{\isundefined{\corollary}}{\newtheorem{corollary}{Corollary}}{}
\ifthenelse{\isundefined{\alg}}{\newtheorem{alg}{Algorithm}}{}
\ifthenelse{\isundefined{\example}}{\newtheorem{example}{Example}}{}
\newcommand\cv{\ensuremath{\to}} % Convergence
\newcommand\cvL{\ensuremath{\xrightarrow{\mathcal{L}}}} % Convergence in law
\newcommand\cvd{\ensuremath{\xrightarrow{d}}} % Convergence in distribution
\newcommand\cvP{\ensuremath{\xrightarrow{P}}} % Convergence in probability
\newcommand\cvas{\ensuremath{\xrightarrow{a.s.}}} % Convergence almost surely
\newcommand\eqdistrib{\ensuremath{\stackrel{d}{=}}} % Equal in distribution
\newcommand{\E}{\ensuremath{\mathbb{E}}} % Expectation
\newcommand\KL[2]{\ensuremath{\text{KL}\left( #1 \| #2 \right)}} % KL-divergence

